Beyond a Million Tokens: Benchmarking and Enhancing Long-Term Memory in LLMs

Evaluating the abilities of large language models (LLMs) for tasks that require long-term memory and thus long-context reasoning, for example in conversational settings, is hampered by the existing benchmarks, which often lack narrative coherence, cover narrow domains, and only test simple recall-oriented tasks. This paper introduces a comprehensive solution to these challenges. First, we present a novel framework for automatically generating long (up to 10M tokens), coherent, and topically diverse conversations, accompanied by probing questions targeting a wide range of memory abilities. From this, we construct BEAM, a new benchmark comprising 100 conversations and 2,000 validated questions. Second, to enhance model performance, we propose LIGHT-a framework inspired by human cognition that equips LLMs with three complementary memory systems: a long-term episodic memory, a short-term working memory, and a scratchpad for accumulating salient facts. Our experiments on BEAM reveal that even LLMs with 1M token context windows (with and without retrieval-augmentation) struggle as dialogues lengthen. In contrast, LIGHT consistently improves performance across various models, achieving an average improvement of 3.5%-12.69% over the strongest baselines, depending on the backbone LLM. An ablation study further confirms the contribution of each memory component.

==> Prompts/add_special_bullets_to_conversation_plan.tex <==
You are a specialized editor that adds three specific test bullets to existing batch plans for synthetic conversation generation.

## INPUT & TASK
- **PLAN:** <plan>
- For EACH batch: Keep ALL <num_bullets> original bullets unchanged, ADD exactly 3 bullets at positions <num_bullets>+1, <num_bullets>+2, <num_bullets>+3

## MANDATORY OUTPUT STRUCTURE
Each batch MUST have EXACTLY <num_bullets>+3 bullets:
- Bullets 1-<num_bullets>: Original bullets (unchanged)
- Bullet <num_bullets>+1: Information Update
- Bullet <num_bullets>+2: User Instruction  
- Bullet <num_bullets>+3: Logical Contradiction

## THE THREE SPECIAL BULLETS
### 1. INFORMATION UPDATE (Bullet <num_bullets>+1)
**Format:** `• **Information Update:** [Natural narrative containing update]`

**MANDATORY PRE-CHECK:**
1. SCAN bullets 1-<num_bullets>-2 for EXPLICIT numerical/measurable data
2. IDENTIFY exact number, time, date, or measurement
3. VERIFY value is clearly stated in original text
4. ONLY THEN create update changing that exact value

EXAMPLES:
[Some examples]

**CRITICAL:** Make update IMPLICIT - embed new value in natural narrative, don't state "X is now Y"

**Update Categories (rotate through all):**
1. Numerical shifts (prices, quantities, measurements)
2. Status changes (employment, relationships, health)
3. Location changes (addresses, venues, destinations)
4. Relationship progressions (social connections)
[Some other categories]

**VERIFICATION:** STOP if no matching fact exists in bullets 1-<num_bullets>-2.

### 2. USER INSTRUCTION (Bullet <num_bullets>+2)
**Format:** `• **User Instruction:** Always [action] when I ask about [condition]`

**MANDATORY FORMAT:** Must include "when I ask about" - this makes it testable.

**Instruction Types (rotate through all):**
1. Output formatting rules
2. Content restrictions
3. Personal preferences
4. Conditional responses
5. Time-based rules
[Some other categories]

**EXAMPLES:**
[Some examples]

### 3. LOGICAL CONTRADICTION (Bullet <num_bullets>+3)
**Format:** `• **Logical Contradiction:** [Contradicting fact only]`

**CRITICAL PRE-CHECK:**
1. SCAN bullets 1-<num_bullets>-2 for COMPLETED ACTIONS or PERMANENT STATES:
   - Past tense actions: "visited", "ate", "traveled", "lived"
   - Permanent conditions: "born in", "raised as", "died in"
   - Absolute statements: "never did X", "always was Y"
2. FIND exactly ONE target fact to contradict
3. IF NO COMPLETED ACTIONS EXIST: CREATE setup bullet with completed action, insert between bullets 5-<num_bullets>-2, THEN contradict in bullet <num_bullets>+4

FORBIDDEN WORDS/PHRASES (NEVER USE):
"Before this batch", "In this batch", [Other examples]

**RULE:** Only contradict COMPLETED ACTIONS, never plans/intentions.

TEMPORAL QUALIFIER PROBLEM:
[Some examples]


FORBIDDEN WORDS/PHRASES (NEVER USE):
"Before this batch", "In this batch", "Previously", 
[Other examples]

**CRITICAL:** Contradiction must make the **same original event/fact IMPOSSIBLE**, not describe a different event with different outcomes.

**Contradiction Types (use variety):**
1. Age/Time Reversal: Age going backward
2. Death Resurrection: Dead people doing activities  
3. Never-Statement Violations: Contradicting "never" claims
4. Location Impossibilities: Being in two places simultaneously
5. Only-Statement Conflicts: Contradicting exclusivity

**VERIFICATION:**
Original is COMPLETED ACTION (past tense)?
Contradiction makes original IMPOSSIBLE, not just different?
Reads like normal, natural statement with NO hint words?
Avoided ALL forbidden words that suggest conflict?

## CRITICAL VERIFICATION STEPS
**Information Update:**
- Can you point to EXACT number/time/date from bullets 1-<num_bullets>-2?
- Changing ONLY that specific value?

**Logical Contradiction:**
- Can you point to EXACT bullet (1-<num_bullets>-2) being contradicted?
- Original fact is COMPLETED ACTION, not plan?
- Contradiction is IMPOSSIBLE, not just different?
- NOT using FORBIDDEN WORDS/PHRASES mentioned in LOGICAL CONTRADICTION section

## COMMON ERRORS TO AVOID
Don't place special bullets anywhere except <num_bullets>+1, <num_bullets>+2, <num_bullets>+3
Don't modify original <num_bullets> bullets
Don't skip any of the three special bullets
Don't use other labels for special bullets

## OUTPUT FORMAT
Return COMPLETE plan where each batch has ALL original bullets unchanged + exactly 3 additional bullets at the end. When setup fact is created, insert between bullets 5-<num_bullets>-2, renumber, and add special bullets as <num_bullets>+2, <num_bullets>+3, <num_bullets>+4.

Begin processing the plan now.

==> Prompts/baseline/kv_creation.tex <==
I provide you with a text. Your task it to identify all the details stated in the text,
and output that in key: value format.
E.g.:
Key 1: Value 1,
Key 2: Value 2,
Key 3: Value 3,
....

Also at the end, I want you to provide a brief summary of what this text was about in this format: Summary: 'summarized text'

Note: only output key-values and the summary. DO NOT provide any explanation before or after that.
Note: Do not output Key 1, Key 2, ...

**Previous Context:**
{history}

text: {text}

==> Prompts/baseline/noise_filtering.tex <==
I provide you with a user query and a text chunk.
You need to decide if the text chunk is nesseccery for answering user question.
If we need the text chunk to answer the user question, or if the text chunk is part of the answer to user question return 'yes'
If the text chunk is noise and not relevant to user question, return 'no'.
Output format: Return only 'yes' or 'no', without any explantion before or after that.

User query: {query} \n\n
Text chunk: {doc_text}

==> Prompts/baseline/rag_answer_generation.tex <==
You are an assistant that MUST answer questions using ONLY the information provided in the context below. 

STRICT INSTRUCTIONS:
1. Answer ONLY based on the provided context
2. Do NOT use your internal knowledge

CONTEXT:
<context>

QUESTION:
<question>

ANSWER REQUIREMENTS:
- Be direct and concise
- Only output the answer to the question without any explanation 

RESPONSE:

==> Prompts/baseline/scratchpad_creation.tex <==
You are a highly analytical AI assistant. Your task is to analyze the latest conversation exchange and produce a structured summary of key information and insights.

**Your Internal Process:**
To ensure maximum accuracy, you must first think step-by-step.
1.  **Analyze:** Break down the user's latest message.
2.  **Identify:** Pinpoint all facts, instructions, and updates.
3.  **Deduce:** Reason about the implications of the new information in the context of the conversation history. What is the user's underlying goal or state?
4.  **Format:** After completing your internal analysis, format the conclusions into the `Extracted Facts` structure.

**Crucial Instruction:** Your final output must **ONLY** be the `Extracted Facts` block. **DO NOT** include your step-by-step reasoning or any other text in your response. Strictly follow the format shown in the example's output.

---
**EXAMPLE**

**Conversation Context:**
* **Recent Conversation History:**
    USER: Hey, I need some help with the "Project Phoenix" launch plan.
    ASSISTANT: Of course. What do you need?
    USER: The launch date is set for September 15th, 2025. I'm responsible for the marketing materials.
* **Latest Exchange to Analyze:**
    USER: Okay, the final budget for the social media campaign is $7,500. The client, Innovate Corp, just approved it. Please find me three case studies of successful B2B SaaS launches by tomorrow, August 28th. And don't include any of our direct competitors in the examples.
    ASSISTANT: Understood. I will find three case studies of successful B2B SaaS launches, excluding competitors, and have them for you by tomorrow, August 28th. The approved budget of $7,500 for the social media campaign has been noted.

**Example of Correct Final Output:**
    * The client's name is "Innovate Corp".
    * The project is related to a "B2B SaaS launch".
    * The final budget for the social media campaign is \$7,500.
    * A deadline is set for "tomorrow, August 28th".
    * User intends to review three case studies for the project.
    * Instruction: Find three case studies.
    * Constraint: Do not include direct competitors in the examples.
    * The budget for the social media campaign has been approved by the client.
    * The user is under a deadline and needs the case studies urgently to inform their work on the marketing materials.

---
**ACTUAL TASK**

**Recent Conversation History:**
{history}

**Latest Exchange to Analyze:**
USER: {latest_user_message}
ASSISTANT: {latest_assistant_message}

**Extracted Facts:**

==> Prompts/baseline/summary_creation.tex <==
You are tasked with summarizing and compressing scratch pad content to fit within a specific token limit.
**Input Content:**
{content}

**Target Length:** {tokens_limit} tokens

**Your Task:**
Compress this content by clustering related information, removing redundancy, and prioritizing the most important details.

**Process:**
1. **Cluster**: Group related information by topic, entity, or theme
2. **Deduplicate**: Remove redundant or repetitive information
3. **Prioritize**: Keep the most important and contextually relevant details
4. **Compress**: Condense while maintaining essential meaning and context

**Output Format:**
Return ONLY the compressed content organized as:

**KEY ENTITIES & RELATIONSHIPS:**
- [Most important people, organizations, systems mentioned]

**CORE DECISIONS & PREFERENCES:**
- [Critical decision points, requirements, constraints]

**PROCESSES & WORKFLOWS:**
- [Essential procedural information and methodologies]

**USER PREFERENCES:**
- [User's stated likes, dislikes, preferred methods, settings, choices]

**USER INSTRUCTIONS:**
- [Specific directions, commands, or guidance provided by the user]

**IMPORTANT DATES:**
- [Deadlines, milestones, scheduled events, time-sensitive information]

**CRITICAL CONTEXT:**
- [Background information necessary for understanding]

**ACTIONABLE ITEMS:**
- [Next steps, pending actions, deadlines]

**IMPORTANT DEVELOPMENTS:**
- [Significant events, changes, milestones]

**Requirements:**
- Stay within {tokens_limit} tokens
- Eliminate redundancy while preserving essential information
- Eliminate older values when there is newer and updated value for a thing
- Maintain chronological context where important
- Prioritize information with ongoing relevance"

**CRITICAL LENGTH REQUIREMENT:**
- Your response should be approximately {tokens_limit} tokens
- If your draft is significantly shorter than {tokens_limit} tokens, ADD MORE DETAIL

==> Prompts/conversation_plan_coding_generation.tex <==
=========== CRITICAL DETAIL REQUIREMENTS ===========
**MANDATORY SPECIFIC DETAILS:**
Every batch MUST include numerous concrete, verifiable technical details that enable single-word or short factual answers:

**Required Detail Categories (minimum 5-7 per batch):**
- **Exact Numbers:** version numbers (v2.3.1), port numbers (3000), response times (250ms), file sizes (2.5MB)
- **Specific Dates/Times:** deployment dates, sprint deadlines, meeting times, build timestamps
- **Named Technologies:** specific frameworks, libraries, tools, services (React 18.2, PostgreSQL 14, AWS Lambda)
- **Error Messages:** exact error texts, status codes (404, 500), stack trace snippets
- **Yes/No Situations:** feature implemented, bug fixed, test passed, deployment successful
- **Performance Metrics:** load times, query speeds, memory usage, API response times
- **Configuration Details:** environment variables, API endpoints, database schemas
- **Quantifiable Results:** test coverage (85%), uptime (99.9%), user count (1,000+), bug count

**Detail Distribution Rules:**
- Each bullet must contain AT LEAST one verifiable technical detail
- Avoid vague statements like "worked on feature" - specify WHAT feature and HOW
- Replace "had a bug" with "encountered 'undefined is not a function' error in UserAuth.js line 42"
- Instead of "improved performance" use "reduced API response time from 800ms to 200ms"

=========== STRUCTURE REQUIREMENTS ===========
TECHNICAL CONTINUITY SYSTEM:**
**Development Phase Evolution:** 
Every technical element MUST show progression from previous batches:

**Natural Development Progression Examples:**
- **Planning Phase:** "I need to design the authentication system..."
[More examples]

**Technical Complexity Progression:**
- Early batches: Basic implementation, simple features
- Middle batches: Integration challenges, debugging complex issues
- Later batches: Performance optimization, advanced features, production concerns

=========== CONFLICT & RESOLUTION TRACKING ===========
**Mandatory Technical Conflict Elements:**
Each batch must include at least 2-3 technical challenges with:
- **Clear Stakes:** what's at risk (deployment deadline, performance SLA, budget constraint)
- **Binary Decisions:** chose Framework A over B, implemented Solution X vs Y, fixed vs workaround
- **Measurable Outcomes:** reduced latency by Xms, saved $X in hosting, improved performance by X%
- **Specific Trade-offs:** what was sacrificed for what gain (memory for speed, complexity for features)

**Technical Conflict Types to Rotate:**
- Performance bottlenecks with specific metrics
- Architecture decisions with concrete alternatives
- Integration challenges with external systems
- Security vulnerabilities with severity levels
- Scalability issues with user load numbers
- Technical debt vs new features

=========== CONTENT DISTRIBUTION STRATEGY ===========
**Per Batch Requirements:**
- 2-3 bullets: Technical implementation details with specific code elements
- 2-4 bullets: Current development status with measurable metrics
- 1 bullet: Exact temporal anchor (specific date/time)
- 5-7 bullets: Development activities with verifiable outcomes
- 3-4 bullets: Technical decisions with specific alternatives considered
- 1 bullet: **Preference Statement**: implicitly showing developer preferences
- Rest: Using remaining labels with concrete technical details

**Adaptive Batch Planning:**
Each batch should organically focus on what makes sense for that development phase:

**Implementation-Heavy Batch:**
- Multiple implementation requests
- Architecture decisions
- Code structure planning
- Framework/library selection

[More examples]

=========== NATURAL CODING CONVERSATION FLOW ===========
Each bullet should represent realistic developer-AI interactions:

**Implementation Requests:**
[Examples]

**Debugging Help:**
[Examples]

**Code Review/Optimization:**
[Examples]

=========== EXECUTION NOTES ===========
- Use plain, technical language throughout
- Include realistic technical specificity: version numbers, error messages, configuration details
- Make every bullet contribute to the overarching development story
- Ensure uniform technical detail quality across ALL batches
- Vary batch focus organically based on development phase (implementation vs debugging vs optimization)
- Prioritize concrete technical details over abstract descriptions
- Every bullet should enable at least 2-3 factual technical questions
- End immediately after `BATCH <num_batches> PLAN`

==> Prompts/conversation_plan_general_generation.tex <==
You are a long-form narrative planning specialist creating a COHERENT STORY PLANSET for natural conversational flow. 
Your task is to generate detailed batch plans that will seed realistic user-assistant dialogue.

## INPUT DATA
- **DOMAIN:** <domain>
- **TITLE:** <title>
- **THEME:** <theme>
- **SUBTOPICS:** <subtopics>
- **TIMELINE:** <timeline>
- **NUM_BATCHES:** <num_batches> batches
- **LABELS:** <provided_labels>
- **USER PROFILE:** <user_profile>
- **USER RELATIONSHIPS:** <user_relationships>

=============== CORE OBJECTIVE ===============
Generate <num_batches> distinct, non-repetitive batch plans that form a coherent narrative arc where a real person naturally converses with an AI assistant. 
Each plan must introduce NEW story elements while maintaining perfect continuity and character consistency.

=============== CRITICAL DETAIL REQUIREMENTS ===============
**MANDATORY SPECIFIC DETAILS:**
Every batch MUST include numerous concrete details that enable factual answers:

**Required Detail Categories (minimum 5-7 per batch):**
- **Exact Numbers:** prices ($X), quantities, percentages, measurements, distances
- **Specific Dates/Times:** For example: "Month x yth", "x:y PM/AM", "next [week day]", "in x weeks", ...
- **Named Locations:** restaurants, stores, streets, buildings, parks, venues
- **Brand/Product Names:** specific items, services, companies, tools, software
- **Yes/No Situations:** decisions made, preferences stated, conflicts resolved
- **Event Outcomes:** what happened, who won/lost, what was chosen/rejected
- **Specific Preferences:** favorite foods, colors, activities, music, books
- **Quantifiable Results:** test scores, rankings, ratings, completion times

**Detail Distribution Rules:**
- Each bullet must contain AT LEAST one verifiable detail
- Avoid vague statements like "discussed options" - specify WHAT options
- Instead of "considering choices" use "choosing between X, Y, and Z"

=============== STRUCTURE REQUIREMENTS ===============
**1. OUTPUT FORMAT:**
- Generate exactly <num_batches> plans
- Format: `BATCH X PLAN` headers
- Each plan contains exactly <num_bullets> bullets
- Each bullet: "• **[LABEL CATEGORY]:[LABEL DESCRIPTION]:** [content]" (<=25 words)
- NOTE: Each label consists of category and description. Use both for each bullet point.
- Use only the provided LABELS - no custom categories
- CRITICAL: Add one time anchor bulletpoint at the begining of each batch with this format: Month Day, Year. 
**NOTE**: Time anchor must correlated with other dates in the batch and the time anchors among batches should be increasing and time anchor in each batch should be before the dates mentioned in the batches.

**2. STORY PROGRESSION ARCHITECTURE:**
**BATCH 1 (Story Foundation):**
- First bullet MUST be: "• **Time Anchor:**"
- Second bullet MUST be: "• **Personal Introduction:**" [Must be from user language (I ...)]
- MUST HAVE one bullet (titled personality trait) from personality_traits in USER PROFILE
- Establish initial context with SPECIFIC details (age, location, job title, salary range)
- Introduce all relationships with CONCRETE contexts (how long known, where met)
- Set up measurable goals, deadlines, and quantifiable challenges

**BATCHES 2-<num_batches> (Story Evolution):**
- Reference user as "I/my/me" (never repeat the full name)
- Each batch advances the timeline chronologically
- Build upon ALL previously established elements
- Show MEASURABLE progression (promotions, relationship milestones, achievement metrics)

**3. RELATIONSHIP CONTINUITY SYSTEM:** [Other details if domain is Coding or Math]
**Relationship Evolution Mandate:**
Every relationship mention MUST include specific interaction details:

**Evolution Stages with Required Details:**
- **Introduction:** "Met [Name] at [specific place] on [date/time]"
- **Development:** "[Name] suggested [specific action] which resulted in [outcome]"
- **Deepening:** "[Name] revealed [specific information] during [specific event]"
- **Maturation:** "After [X months/years], [Name] and I [specific change]"

**Interaction Variety (rotate - never repeat within batches):**
- Collaborative, Supportive, Conflictual, Social, Professional, Personal, Transactional, Serendipitous

**Character Consistency Rules:**
- Track specific preferences for each character (favorite restaurant, hobby, pet peeve)
- Reference past specific events and their measurable consequences
- Include 2-3 relationship bullets per batch with concrete details

=============== CONFLICT & RESOLUTION TRACKING ===============
**Conflict Elements:**
Each batch must include situations with:
- **Binary Decisions:**
- **Measurable Outcomes:**
- **Specific Disagreements:**

**Conflict Types to Rotate:**
- Financial decisions with specific amounts
- Time management with exact deadlines
- Relationship boundaries with specific incidents
- Professional choices with concrete options
- Personal values with specific scenarios

=============== ANTI-REPETITION VERIFICATION ===============
**Before writing ANY bullet, verify:**
- Have I included at least one specific, verifiable detail?
- Can this generate a question with a one-word answer?
- Does this show MEASURABLE progression from previous mentions?
- Are the numbers, dates, names, and locations specific?
- Is this a NEW piece of information with NEW details?

=============== CONTENT DISTRIBUTION STRATEGY ===============
**Per Batch Requirements:**
- 2-3 bullets: Relationship developments with specific incidents
- 2-4 bullets: Current situation with measurable metrics
- 1 bullet: Exact temporal anchor (specific date/time)
- 5-7 bullets: Events with verifiable outcomes
- 3-4 bullets: Decisions/preferences with specific choices
- 1 bullet: **Preference Statement**: implicitly showing user preferences
- Rest: Using remaining labels with concrete details

=============== SPECIAL BULLET REQUIREMENTS ===============
**1. PREFERENCE STATEMENT (rotate each batch):**
Must show preference through action/decision

**Rotate These Types Each Batch:**
- Choice actions
- Method implementations
- Quality decisions
- Timing patterns
- Style approaches
- Priority demonstrations

**Story Progression Patterns:**
- **Early Batches (1-3):** Establish baselines (current salary, relationship status, living situation)
- **Middle Batches:** Track changes from baselines with specific metrics
- **Later Batches:** Show cumulative results with before/after comparisons

=============== QUALITY STANDARDS ===============
**Specificity Checklist:**
- Every person has a full name and defined relationship
- Every event has a date, time, or specific temporal reference
- Every location has a name or address
- Every decision has concrete options with specific details
- Every outcome is measurable or verifiable

**Narrative Depth:**
- Include prices, percentages, distances, durations
- Show cause-and-effect with specific triggers and results
- Maintain factual consistency (don't change established numbers/dates)
- Reference past specific events by name and date

=============== EXECUTION NOTES ===============
- Prioritize concrete details over abstract descriptions
- Every bullet should enable at least 2-3 factual questions
- Include cultural, financial, and geographic specificity
- Ensure details are realistic and internally consistent
- End immediately after `BATCH <num_batches> PLAN`

Begin generation now.

==> Prompts/conversation_plan_math_generation.tex <==
=========== CRITICAL DETAIL REQUIREMENTS ===========
**MANDATORY SPECIFIC DETAILS:**
Every batch MUST include numerous concrete, verifiable mathematical details that enable single-word or short factual answers:

**Required Detail Categories (minimum 5-7 per batch):**
- **Exact Numbers:** specific values (x = 3.14), coefficients ($2x^2 + 5x - 3$), dimensions ($5\times7$ matrix)
- **Specific Problems:** complete equations ($x^2 - 4x + 3 = 0$), specific integrals ($\int_0^5 (2x+1)\,dx$)
- **Named Concepts:** theorem names (Pythagorean Theorem), method names (Gaussian elimination), formulas (quadratic formula)
- **Calculation Results:** exact answers ($x = 4$), decimal results ($\pi \approx 3.14159$), fractions ($\tfrac{3}{4}$)
- **Yes/No Situations:** problem solved correctly, method applicable, theorem satisfied, solution exists
- **Score/Grade Metrics:** test scores (85%), homework grades (18/20), quiz results (9/10 correct)
- **Time/Duration:** study hours (3 hours), problem completion time (15 minutes), exam duration (2 hours)
- **Mathematical Properties:** function characteristics (continuous, differentiable), matrix properties (invertible, symmetric)

**Detail Distribution Rules:**
- Each bullet must contain AT LEAST one verifiable mathematical detail
- Avoid vague statements like "worked on problems" - specify WHICH problems and results
- Replace "studied math" with "completed 5 quadratic equation problems, solved 4 correctly"
- Instead of "improved understanding" use "increased quiz score from 70% to 85%"

=============== STRUCTURE REQUIREMENTS ===============
**3. MATHEMATICAL CONTINUITY SYSTEM:**
**Learning Phase Evolution:** 
Every mathematical element MUST show progression from previous batches:

**Natural Learning Progression Examples:**
- **Conceptual Phase:** "I need to understand what derivatives mean..."
[More examples]

=============== CONFLICT & RESOLUTION TRACKING ===============
**Mandatory Mathematical Conflict Elements:**
Each batch must include at least 2-3 mathematical challenges with:
- **Clear Stakes:** what's at risk (exam grade, assignment deadline, course prerequisite)
- **Binary Decisions:** chose Method A over B, applied Theorem X vs Y, used algebraic vs geometric approach
- **Measurable Outcomes:** improved accuracy by X%, reduced solution time by Y minutes, raised grade from B to A
- **Specific Struggles:** which step caused confusion, what concept was misunderstood, where calculation went wrong

**Mathematical Conflict Types to Rotate:**
- Conceptual misunderstandings with specific confusion points
- Calculation errors with exact mistake locations
- Method selection dilemmas with pros/cons
- Time pressure challenges with specific deadlines
- Prerequisite knowledge gaps with missing concepts
- Application difficulties with real-world connections

=============== CONTENT DISTRIBUTION STRATEGY ===============
**Per Batch Requirements:**
- 2-3 bullets: Problem-solving activities with specific equations/solutions
- 1-2 bullets: Current learning status with measurable metrics
- 1 bullet: Exact temporal anchor (specific date/time)
- 4-6 bullets: Mathematical activities with verifiable outcomes
- 2-3 bullets: Learning decisions with specific alternatives considered
- 1 bullet: **Preference Statement**: implicitly showing learning preferences
- Rest: Using remaining labels with concrete mathematical details

**Adaptive Batch Planning:**
Each batch should organically focus on what makes sense for that learning phase:

[More examples]

=============== NATURAL MATH CONVERSATION FLOW ===============
Each bullet should represent realistic user-AI interactions:

**Problem-Solving Requests:**
[examples]

**Concept Clarification:**
[examples]

**Solution Verification:**
[examples]

**Method Explanation:**
[examples]

=============== QUALITY STANDARDS ===============

**Chronological Consistency:**
- Batch 1 = learning beginning/foundation phase
- Batch <num_batches> = evolved understanding with clear mathematical progression
- Each batch logically follows the previous learning timeline

**Mathematical Authenticity:**
- Include specific mathematical details: equation types, theorem names, calculation methods
[More examples]

**User Authenticity:**
- Keep user personality consistent with provided profile
[More examples]

**Learning Realism:**
- Follow realistic mathematical learning patterns
[More examples]

**Specificity Checklist:**
- Every equation has specific coefficients and variables
[More examples]

=============== EXECUTION NOTES ===============

- Use plain, mathematical language throughout
- Include realistic mathematical specificity: complete equations, exact values, specific theorems
- Make every bullet contribute to the overarching mathematical story
- Ensure uniform mathematical detail quality across ALL batches
- Vary batch focus organically based on learning phase (understanding vs solving vs applying)
- Prioritize concrete mathematical details over abstract descriptions
- Every bullet should enable at least 2-3 factual mathematical questions
- End immediately after `BATCH <num_batches> PLAN`

Begin generation now.

==> Prompts/llm_as_a_judge_prompt.tex <==
You are an expert evaluator tasked with judging whether the LLM's response demonstrates compliance with the specified RUBRIC CRITERION.

## EVALUATION INPUTS
- QUESTION (what the user asked): <question>
- RUBRIC CRITERION (what to check): <rubric_item>
- RESPONSE TO EVALUATE: <llm_response>

## EVALUATION RUBRIC:
The rubric defines a specific requirement, constraint, or expected behavior that the LLM response should demonstrate. 

**IMPORTANT**: Pay careful attention to whether the rubric specifies:
- **Positive requirements** (things the response SHOULD include/do)
- **Negative constraints** (things the response SHOULD NOT include/do, often indicated by "no", "not", "avoid", "absent")

## RESPONSIVENESS REQUIREMENT (anchored to the QUESTION)
A compliant response must be **on-topic with respect to the QUESTION** and attempt to answer it.
- If the response does not address the QUESTION, score **0.0** and stop.
- For negative constraints, both must hold: (a) the response is responsive to the QUESTION, and (b) the prohibited element is absent.

## SEMANTIC TOLERANCE RULES:
Judge by meaning, not exact wording.
- Accept **paraphrases** and **synonyms** that preserve intent.
- **Case/punctuation/whitespace** differences must be ignored.
- **Numbers/currencies/dates** may appear in equivalent forms (e.g., “$68,000”, “68k”, “68,000 USD”, or “sixty-eight thousand dollars”). Treat them as equal when numerically equivalent.
- If the rubric expects a number or duration, prefer **normalized comparison** (extract and compare values) over string matching.

## STYLE NEUTRALITY (prevents style contamination):
Ignore tone, politeness, length, and flourish unless the rubric explicitly requires a format/structure (e.g., “itemized list”, “no citations”, “one sentence”).
- Do **not** penalize hedging, voice, or verbosity if content satisfies the rubric.
- Only evaluate format when the rubric **explicitly** mandates it.

## SCORING SCALE:
- **1.0 (Complete Compliance)**: Fully complies with the rubric criterion.
  - Positive: required element present, accurate, properly executed (allowing semantic equivalents).
  - Negative: prohibited element **absent** AND response is **responsive**.
  
- **0.5 (Partial Compliance)**: Partially complies.
  - Positive: element present but minor inaccuracies/incomplete execution.
  - Negative: generally responsive and mostly avoids the prohibited element but with minor/edge violations.
  
- **0.0 (No Compliance)**: Fails to comply.
  - Positive: required element missing or incorrect.
  - Negative: prohibited element present **or** response is non-responsive/evasive even if the element is absent.

## EVALUATION INSTRUCTIONS:
1. **Understand the Requirement**: Determine if the rubric is asking for something to be present (positive) or absent (negative/constraint).

2. **Parse Compound Statements**: If the rubric contains multiple elements connected by "and" or commas, evaluate whether:
   - **All elements** must be present for full compliance (1.0)
   - **Some elements** present indicates partial compliance (0.5)
   - **No elements** present indicates no compliance (0.0)
   
3. **Check Compliance**: 
   - For positive requirements: Look for the presence and quality of the required element
   - For negative constraints: Look for the absence of the prohibited element

4. **Assign Score**: Based on compliance with the specific rubric criterion according to the scoring scale above.

5. **Provide Reasoning**: Explain whether the rubric criterion was satisfied and justify the score.

## OUTPUT FORMAT:
Return your evaluation in JSON format with two fields:

{
   "score": [your score: 1.0, 0.5, or 0.0],
   "reason": "[detailed explanation of whether the rubric criterion was satisfied and why this justified the assigned score]"
}

NOTE: ONLY output the json object, without any explanation before or after that

==> Prompts/llm_equivalence_detector.tex <==
You are a binary classifier.
If the TWO snippets describe the SAME event/fact, reply **YES**
Otherwise reply **NO**. No extra words.
DO NOT provide any explanation.

First snippet: {first_paragraph}
Second snippet: {second_paragraph}

==> Prompts/narrative_generation.tex <==
You are a conversation framework specialist tasked with identifying the most relevant section label categories for a specific chat scenario.

INPUT PARAMETERS:
DOMAIN: {}
TITLE: {}
THEME: {}
SUBTOPICS: {}

CORE OBJECTIVE:
Analyze the given DOMAIN, TITLE, THEME, SUBTOPICS to determine which section label categories would be most relevant and natural for this specific scenario. 
Generate 15-20 section label categories that best fit this particular context.

LABEL CATEGORIES SELECTION:
Here are some examples:

**UNIVERSAL CATEGORIES (Always Include 2-3):**
- **Character & Relationship Labels** (relationships are always relevant)
- **Personal & Emotional Labels** (human element always present)
- **Decision & Change Labels** (conversations involve decisions)

**TOPIC-SPECIFIC CATEGORIES (Select 9-13 based on relevance):**

**Planning & Logistics Labels** - Use when scenario involves:
- Travel, events, projects, moves, construction, organizing
- Resource management, scheduling, coordination
- Physical planning or systematic approaches

[More examples]

ELECTION CRITERIA:
**Must Include If Relevant:**
- Categories directly related to the main topic
- Categories that would naturally generate diverse conversations
- Categories that allow for progression and development over time
- Categories that create authentic human concerns and interests

**Avoid Including:**
- Categories that don't naturally fit the scenario
- Too many similar categories that would overlap
- Categories that wouldn't generate meaningful conversation
- Generic categories that don't add specific value

OUTPUT FORMAT:
Generate exactly 15-20 section label categories in this format:

**[Category Name] Labels:**
- Brief explanation of why this category is relevant to the DOMAIN/TITLE/THEME/SUBTOPICS
- 3-5 specific label examples that would be used within this category

Example:
**Planning & Logistics Labels:**
- Essential for travel scenarios involving coordination, scheduling, and resource management
- Budget Planning, Transportation Strategy, Accommodation Research, Itinerary Adjustment, Packing Organization

QUALITY STANDARDS:
Each selected category must:
- Be directly relevant to the specific DOMAIN, TITLE and THEME
- Generate natural, varied conversation opportunities  
- Allow for progression and development across multiple batches
- Feel authentic to what a real person would discuss in this scenario
- Provide enough depth for 15-20 bullet points across the conversation
- Just ouput the labels, without explanation at the first

Focus on categories that would create the most natural, engaging, and realistic chat conversations for this specific scenario.

==> Prompts/probing_questions/abstention_generation.tex <==
You are tasked with generating multiple probing questions to test abstention capabilities of LLMs. You will be given a plan containing bullet points that will be used to generate conversations between a user and AI assistant.

Your task is to create questions that test whether an LLM can appropriately respond with "I don't know" or "Based on the provided chat, there is no information related to [topic]" when asked about information that is missing or unavailable from the plan.

## INPUT DATA
- **PLAN**: <plan>

## CRITICAL REQUIREMENT: EARLY BATCH PRIORITIZATION
**SELECTION PRIORITY ORDER:**
1. **Batch 1-3 (HIGHEST PRIORITY)**: Select 70-80% of your questions from these early batches
2. **Batch 4-6 (MEDIUM PRIORITY)**: Select 10-20% of your questions from these middle batches  
3. **Batch 7+ (LOW PRIORITY)**: Select only 5-10% of your questions from later batches

## CRITICAL REQUIREMENT: CONTEXT-BASED HARD QUESTIONS
- Questions MUST be related to the plan's context and domain
- Ask about plausible information that SEEMS like it should be available but isn't
- Use names, places, events, and topics mentioned in the plan
- Ask for specific details about mentioned entities that aren't actually provided
- Create questions that would be natural follow-ups but can't be answered

## QUESTION GENERATION GUIDELINES
Focus on creating questions that test appropriate abstention for:
### 1. Missing Details About Mentioned People/Entities [Exmaples]
### 2. Unavailable Specifics About Mentioned Events/Activities [Examples]
### 3. Missing Information About Referenced Sources/Materials [Examples]
### 4. Unavailable Details About Mentioned Processes/Procedures [Examples]
### 5. Missing Context About Mentioned Decisions/Choices [Examples]
### 6. Unavailable Quantitative/Measurement Details [Examples]
### 7. Missing Emotional/Subjective Information [Examples]
### 8. Unavailable Technical/Specialized Details [Examples]
### 9. Unavailable Future/Predictive Information [Examples]

## ABSTENTION QUESTION TYPES
Only generate these two types: 1. **Unavailable Information Questions**: Ask about topics, people, events, or details that are completely absent from the plan
2. **Missing Detail Questions**: Ask for specific details about topics that may be mentioned generally but lack the requested specifics

## DIFFICULTY LEVELS
Generate questions of varying abstention difficulty:
- **Easy**: Ask for details about mentioned entities that seem like they should be available
- **Medium**: Ask for specific information about mentioned processes/events that weren't detailed
- **Hard**: Ask for nuanced details that are plausible but not provided

## QUESTION LANGUAGE REQUIREMENTS
- Write questions as if the USER is asking them naturally
- **If testing information from USER messages**: Use first person ("I", my", "me") in question -> Answer uses ("you", "your")
  - Example: "How did I decide on the location?" -> "You decided on the location because..."
- **If testing information from ASSISTANT messages**: Use second person ("you", "your") in question -> Answer uses ("I", "my") 
  - Example: "What steps did you suggest for handling this?" -> "I suggested doing..."
- Avoid phrases like "according to the conversation", "based on what was discussed", "from our chat history"
- Make questions sound conversational and natural
- Questions should flow naturally as if continuing the conversation

## OUTPUT FORMAT
Return your analysis in this exact JSON format:
[{"question": "", "ideal_response": "", "difficulty": "easy", "abstention_type": "", "why_unanswerable": "",
        "plan_reference": ""},
]

## IMPORTANT REQUIREMENTS
1. **Context-based questions**: Questions must relate to plan content and use mentioned entities
2. **Plausible but unavailable**: Ask for information that seems reasonable but isn't provided
3. **Natural follow-ups**: Questions should sound like logical next questions about mentioned topics
4. **Challenging abstention**: Make it harder for LLM to recognize information is missing
5. **Domain consistency**: Questions should fit naturally within the plan's subject matter

Generate 8-15 abstention questions that test the LLM's ability to appropriately say "Based on the provided chat, there is no information related to [topic]" when information is missing or unavailable in the plan.

NOTE: Only output the JSON array without any explanation before or after the list.

==> Prompts/probing_questions/contradiction_resolution.tex <==
This is a plan that contains detailed bullet points about a topic. This plan is used to generate realistic chat conversations between a user and an AI assistant, which are then used to evaluate the long-term memory capabilities of LLMs. 
Your task is to analyze this plan and select PAIRS of bullet points that would be most effective for testing contradiction resolution abilities when incorporated into chat conversations.
Contradiction resolution tests whether the LLM can detect and appropriately handle impossible contradictions - statements that logically cannot both be true simultaneously.
Analyze this project plan and identify PAIRS of bullet points where one completely contradicts the other with impossible contradictions. Each pair should contain statements that are logically incompatible and cannot both be true.

## INPUT DATA
- **PLAN**: <plan>

Focus on bullet point pairs that show:
- **Never-Statement Violations**: One bullet says "never" did something, another shows they did it
- **Always-Statement Violations**: One bullet claims "always" pattern, another breaks that pattern  
- **Only-Statement Conflicts**: One bullet claims exclusivity ("only"), another contradicts it
- **Impossible Reversals**: Age going backward, timeline impossibilities, logical reversals
- **Dead-Alive Contradictions**: References to deceased people being active
- **Mutually Exclusive States**: Being in two places simultaneously, having contradictory capabilities
- **Absolute Negations**: Claiming something is impossible then showing it happened

**Types of Impossible Contradictions to look for:**
1. **Never-Statement Violations**: "Never attended X" vs "Attended X event"
2. **Always-Statement Violations**: "Always lived in Y" vs "Moved from Z to Y"  
3. **Only-Statement Conflicts**: "Only child" vs "Has siblings"
4. **Timeline Impossibilities**: Events happening in wrong chronological order
5. **Capability Contradictions**: "Cannot do X" vs "Successfully did X"
6. **Location Impossibilities**: Being in two places at once
7. **Relationship Contradictions**: "Never met person" vs "Long friendship with person"

Prioritize bullet point pairs that:
- Contain completely impossible contradictions that cannot be resolved or explained
- Use absolute language ("never," "always," "only," "impossible," "cannot")
- Create clear logical impossibilities rather than simple inconsistencies
- Enable questions about detecting fundamental contradictions
- Test whether the AI can identify when statements are mutually exclusive
- Focus on contradictions that are objectively impossible, not subjective differences

Return your analysis in this exact JSON format where each object contains exactly TWO contradicting bullet points:
[{"capability": "contradiction_resolution", "batch_numbers": "1, 8", "bullet_numbers": "30, 29",
        "bullet_points": "• **Logical Contradiction:** Jeremiah has never attended any Bahrain Jazz Festival events. | • **Character & Relationship:Close Friend:** Jeremiah, 37, met at Bahrain Jazz Festival 2015, recommended an acoustic consultant."}
]

Important formatting notes:
- The "batch_numbers" and "bullet_numbers" correspond to each other positionally
- "1, 8" and "30, 29" means: Batch 1 Bullet 30, Batch 8 Bullet 29
- Each object must contain exactly 2 bullet points separated by " | "
- Use comma-separated values for batch_number and bullet_number
- First bullet point can be the contradiction marker or the contradicted statement
- Second bullet point should directly contradict the first with impossible logic
- Focus on pairs that test detection of fundamental logical impossibilities

Select <bullet_number> pairs of bullet points that demonstrate the clearest impossible contradictions for testing contradiction resolution abilities.

NOTE: Only output the list without any explanation before or after the list.

==> Prompts/probing_questions/contradiction_resolution_generation.tex <==
You are tasked with generating a probing question to test contradiction resolution capabilities of LLMs. You will be given two contradictory bullet points and the corresponding multi-turn dialogs between a user and assistant that incorporate both contradictory statements across different conversation sessions.

Your task is to create ONE question that asks about the contradicted topic as if seeking factual information, testing whether the LLM will detect the contradiction and ask for clarification rather than giving a definitive answer.

## INPUT DATA
- **BULLET POINTS**: <bullet_points>
- **CONVERSATION TURNS**: <conversation_turns>

## QUESTION GENERATION GUIDELINES
Focus on creating questions that:
- **Ask about the contradicted fact**: Question the topic that has contradictory information
- **Sound like normal fact-seeking**: Don't hint that there's a contradiction
- **Test contradiction detection**: Whether LLM notices conflicting information
- **Expect clarification request**: LLM should ask which contradictory statement is correct
- **Avoid revealing the contradiction**: Question should seem like routine information request

## CRITICAL REQUIREMENT:
- The question MUST be general and broad about the contradicted topic
- Do NOT include specific dates, times, locations, or detailed circumstances
- Do NOT reference specific events or instances that would narrow down the contradiction
- Ask about the general pattern/behavior, not specific occurrences
- This tests whether the LLM can detect contradictions across all related mentions

## QUESTION LANGUAGE REQUIREMENTS
- Write questions as if the USER is asking them naturally
- Use first person ("I", "my", "me") when referring to the user
- Use second person ("you") when addressing the assistant
- Avoid phrases like "according to the conversation", "based on what was discussed", "from our chat history"
- Make questions sound conversational and natural
- Questions should flow naturally as if continuing the conversation

## QUESTION FORMAT Generate questions that ask about the contradicted topic directly: [Examples]

## EXPECTED LLM BEHAVIOR The ideal LLM response should: [Example]

## CHAT ID TRACKING REQUIREMENT
- You MUST identify which specific chat_id(s) contain each contradictory statement
- List the chat_id for the first contradictory statement and the chat_id for the second contradictory statement
- NOTE: If the answer is spread out between multiple chat_ids, group them in one list
- NOTE: DO NOT INCLUDE chat_ids in the answer
- Use the exact chat_id numbers from the conversation turns

## OUTPUT FORMAT
Return your analysis in this exact JSON format:
{
    "question": "", "ideal_answer": "", "difficulty": "", "contradiction_type": "", "topic_questioned": "", "conversation_references": [],
    "tests_for": "", "source_chat_ids": {"first_statement": [, ], "second_statement": [, ]}
}

## IMPORTANT REQUIREMENTS
1. **Natural question phrasing**: Question should sound like normal fact-seeking, not contradiction testing
2. **Topic focus**: Ask directly about the contradicted subject
3. **Contradiction detection expectation**: LLM should notice and ask for clarification
4. **No hint giving**: Don't reveal that there's a contradiction in the question
5. **Clarification seeking**: Ideal response should ask which statement is correct

Generate ONE contradiction resolution question that tests whether the LLM will detect the contradiction and appropriately request clarification when asked about the contradicted topic.

CRITICAL NOTE: Do NOT include specific dates, times, locations, or detailed circumstances in the question that make the question easy.
NOTE: Only output the JSON object without any explanation before or after.

==> Prompts/probing_questions/event_ordering.tex <==
This is a plan that contains detailed bullet points about a topic. This plan is used to generate realistic chat conversations between a user and an AI assistant, which are then used to evaluate the long-term memory capabilities of LLMs. 
Your task is to analyze this plan and select GROUPS of related bullet points that would be most effective for testing event ordering abilities when incorporated into chat conversations.
Event ordering tests whether the LLM can recall the chronological order in which events or topics were MENTIONED in the conversation, regardless of when the actual events occurred in real life.
Analyze this plan and identify GROUPS of 8-12 or more related bullet points that represent the same topic/theme mentioned across different batches, enabling testing of mention-order recall and conversation sequence understanding.

## INPUT DATA
- **PLAN**: <plan>

## CRITICAL REQUIREMENT: EARLY BATCH PRIORITIZATION
**SELECTION PRIORITY ORDER:**
1. **Groups starting in Batches 1-3 (HIGHEST PRIORITY)**: Select 70-80% of your groups with first mention in early batches
2. **Groups spanning early to middle batches (MEDIUM PRIORITY)**: Select 10-20% of groups that bridge early-to-middle timeline
3. **Groups from later batches only (LOW PRIORITY)**: Select only 5-10% from purely later batches

Focus on bullet point groups that show:
- **Same person mentioned multiple times**: Different interactions or mentions of the same person across batches
- **Same component/process discussed repeatedly**: Multiple mentions of the same equipment, material, or process
- **Same location/venue referenced**: Multiple mentions of the same place or address
- **Same decision/topic revisited**: The same subject brought up in different conversation sessions
- **Same problem/solution mentioned**: Multiple references to the same issue across different times
- **Same financial item tracked**: Multiple mentions of the same cost, budget item, or expense

Prioritize bullet point groups that:
- Contain 8-12 mentions of the same topic across different batches
- Enable questions about "In what order events X,Y,Z,... happen?" Or ...
- Allow testing of conversation chronology rather than real-world event chronology  
- Test recall of mention sequence: "Which did I talk about first, second, third?"
- Focus on the order topics appeared in conversation, not when events actually happened
- Create opportunities to test conversational memory rather than factual timeline memory

Return your analysis in this exact JSON format where each object contains 3+ bullet points about the same topic across different batches:
[{"capability": "event_ordering", "batch_numbers": "1, 3, 5, 7", "bullet_numbers": "22, 18, 11, 27",
        "bullet_points": "• **Character & Relationship:Acoustic Consultant:** Met Rami Al-Hassan at Bahrain Acoustic Expo on Feb 20; he recommended HVAC silencing at $2,200. | • **Character & Relationship:Acoustic Consultant:** Rami conducted mid-project site visit April 3, advised on bass trap repositioning to improve 5 dB absorption. | • **Character & Relationship:Acoustic Consultant:** Rami praised progress in May 1 email; suggested minor EQ tweaks. | • **Character & Relationship:Acoustic Consultant:** Rami praised final results August 20; recommended ongoing maintenance and periodic EQ checks."}
]

Important formatting notes:
- The "batch_numbers" and "bullet_numbers" correspond to each other positionally
- "1, 2, 3, 5, 7" and "22, 18, 11, 27" means: Batch 1 Bullet 22, Batch 3 Bullet 18, Batch 5 Bullet 11, Batch 7 Bullet 27
- Each object must contain 8-12 related bullet points separated by " | "
- Use comma-separated values for batch_number and bullet_number  
- All bullet points must reference the same topic/person/component/theme
- Focus on groups that enable mention-order questions
- Test conversational chronology, not real-world event chronology

Select 8-10 groups of bullet points that would enable the most sophisticated mention-order and conversation sequence questions.

CRITICAL NOTE: DO NOT consider bulletpoint names for selecting the bullets. ONLY consider the bullets contents.
NOTE: Only output the list without any explanation before or after the list.

==> Prompts/probing_questions/event_ordering_generation.tex <==
You are tasked with generating a probing question to test event ordering capabilities of LLMs. You will be given multiple related bullet points about the same topic/theme and the corresponding multi-turn dialogs between a user and assistant that incorporate these mentions across different conversation sessions.

Your task is to create ONE question that tests whether an LLM can recall the chronological order in which topics were MENTIONED in the conversation, regardless of when the actual events occurred in real life.

## INPUT DATA
- **BULLET POINTS**: <bullet_points>
- **CONVERSATION TURNS**: <conversation_turns>

## CRITICAL REQUIREMENTS: NO SPOILERS OR TIME HINTS
- The question MUST NOT list, mention, or hint at the specific events/mentions being tested
- The question should only specify the general topic/theme, not the individual events
- Do NOT include any time references, dates, or temporal hints in the question
- The LLM must recall and order the mentions entirely from memory without any hints

## ADVANCED QUESTION TYPES FOR EVENT ORDERING
### **Sequential Ordering Questions** 1. **General Mention Order** [Other types]
### **Comparative Ordering Questions** 4. **Priority Sequencing** [Other types]
### **Pattern Recognition Questions** 7. **Mention Pattern**: [Other types]
### **Analytical Ordering Questions** 10. **Chronological Reconstruction** [Other types]
### **Complex Sequencing Questions** 13. **Multi-faceted Ordering** [Other types]

## FORBIDDEN QUESTION ELEMENTS
- Do NOT list specific events like "including X, Y, and Z"
- Do NOT mention specific details, dates, times, or temporal references
- Do NOT provide hints about what mentions to look for
- Do NOT reference specific timeframes (e.g., "in February", "during spring", "early in project")
- Do NOT use temporal words like "first", "then", "after", "before" in the question

## GOOD VS BAD EXAMPLES
[Examples]

## ORDERING COMPLEXITY LEVEL: HARD
- **Hard**: Either 8-10 mentions requiring chronological reconstruction or 8-10 mentions with complex conversational patterns or 8+ mentions requiring sophisticated sequence analysis
- Focus on advanced sequence reconstruction with sophisticated analysis
- Test ability to track complex mention patterns across multiple sessions
- Include scenarios requiring expert-level sequence analysis and pattern recognition

## QUESTION LANGUAGE REQUIREMENTS
- Write questions as if the USER is asking them naturally
- Use first person ("I", "my", "me") when referring to the user
- Use second person ("you") when addressing the assistant
- Avoid phrases like "according to the conversation", "based on what was discussed", "from our chat history"
- Make questions sound conversational and natural
- Questions should flow naturally as if continuing the conversation
- NEVER include temporal references or time-related words

## MANDATORY QUESTION ENDING REQUIREMENT
- ALL questions MUST end with the phrase "in order" if previously didn't mention the order
- The order should mention ONLY ONCE
- This signals to the LLM that a sequential, ordered response is expected

## CHAT ID TRACKING REQUIREMENT [ONLY for source_chat_ids filed in JSON object]
- You MUST identify which specific chat_id(s) contain each mention in the ordering sequence
- List ALL chat_ids for each mention in chronological order in source_chat_ids field
- NOTE: If the answer is spread out between multiple chat_ids, group them in one list
- NOTE: DO NOT INCLUDE chat_ids in the answer
- Use the exact chat_id numbers from the conversation turns
- Map each mention to its source chat_id

## OUTPUT FORMAT
Return your analysis in this exact JSON format:
{
    "question": "", "answer": "", "difficulty": "hard", "ordering_type": "", "total_mentions": , "conversation_references": [],
    "ordering_tested": [], "complexity_factors": [], "source_chat_ids": []
}

## IMPORTANT REQUIREMENTS
1. **No temporal hints**: Question must NOT include any time references or temporal words
2. **High question variety**: Use diverse question types from the 15 categories provided
3. **Complex reasoning**: Require sophisticated mention-order analysis
4. **Pattern focus**: Test understanding of conversational patterns and evolution
5. **Advanced difficulty**: Always use "hard" difficulty level
6. **General topic focus**: Ask about broad themes, not specific events
7. **Sophisticated analysis**: Test expert-level sequence reconstruction and pattern recognition

Generate ONE high-quality, challenging event ordering question that tests sophisticated mention-sequence analysis without providing any hints about the specific events or timing.

NOTE: Only output the JSON object without any explanation before or after.

==> Prompts/probing_questions/information_extraction.tex <==
This is a plan that contains detailed bullet points about a topic. This plan is used to generate realistic chat conversations between a user and an AI assistant, which are then used to evaluate the long-term memory capabilities of LLMs. 
Your task is to analyze this plan and select bullet points that would be most effective for testing information extraction abilities when incorporated into chat conversations.
Analyze this plan and identify bullet points that contain specific factual information ideal for testing precise recall and information extraction capabilities.

## INPUT DATA
- **PLAN**: <plan>

## CRITICAL REQUIREMENT: EARLY BATCH PRIORITIZATION
**SELECTION PRIORITY ORDER:**
1. **Batch 1-3 (HIGHEST PRIORITY)**: Select 70-80% of your choices from these early batches
2. **Batch 4-6 (MEDIUM PRIORITY)**: Select 10-20% of your choices from these middle batches  
3. **Batch 7+ (LOW PRIORITY)**: Select only 5-10% of your choices from later batches

Focus on bullet points with:
- **Specific numbers, quantities, measurements, prices, percentages**
- **Proper names of people, organizations, brands, locations**
- **Exact dates, times, schedules, or deadlines**
- **Contact details such as addresses, phone numbers, email IDs**
- **Technical or detailed descriptions (model names, product codes, ratings, specifications)**
- **Distinctive events, awards, or milestones**
- **Direct quotes, messages, or instructions with exact wording**
- **Precise parameters, formulas, or datasets in technical and academic contexts**
- **Mathematical expressions, theorems, proofs**

Prioritize information that:
- Appears early in the timeline
- Contains multiple distinct factual details in one bullet point
- Includes uncommon names, technical terms, or culturally specific references
- Has precise numerical values or measurements that could be easily confused
- Could be misremembered if details are swapped, rounded, or reworded
- Requires high accuracy to preserve meaning (e.g., formulas, addresses, step-by-step processes)

Return your analysis in this exact JSON format:
[{"capability": "information_extraction", "batch_numbers": 1, "bullet_numbers": 3,
        "bullet_points": "• **Personal Introduction:** I am Sherry Rodriguez, 34, licensed conveyancer in Hollyborough, Bahrain, earning approximately $68,000 annually."}
]

Important formatting notes:
- The "batch_numbers" and "bullet_numbers" correspond to each other positionally
- "1" and "3" means: Batch 1 Bullet 3

Select ONLY <bullet_number> bullet points total that would generate the highest quality information extraction questions.

NOTE: Only output the list without any explanation before or after the list.

==> Prompts/probing_questions/information_extraction_hard_generation.tex <==
You are tasked with generating a probing question to test information extraction capabilities of LLMs. You will be given a bullet point and the corresponding multi-turn dialog between a user and assistant that incorporates this bullet point information.

Your task is to create ONE question that tests whether an LLM can precisely extract and recall specific factual details from the conversation through indirect questioning that requires synthesizing multiple details from different parts of the conversation.

## INPUT DATA
- **BULLET POINT**: <bullet_point>
- **CONVERSATION TURNS**: <conversation_turns>

## CRITICAL REQUIREMENT: INFORMATION EXTRACTION
- The question MUST NOT directly ask for the information being tested
- Ask about related topics/contexts that require the LLM to synthesize multiple details from different conversation parts
- Force the LLM to extract and combine information scattered across different conversation turns
- Make the LLM demonstrate knowledge of facts without being directly asked for them
- Require connecting and integrating information from multiple different conversation elements
- Remove ALL specific details from the question that would give away the answer

## FORBIDDEN QUESTION ELEMENTS
- Do NOT repeat specific names, numbers, or details being tested
- Do NOT mention key characteristics or attributes being extracted
- Do NOT include descriptive words that hint at the answer
- Do NOT reference specific categories or types being tested
- Do NOT use qualifying details that narrow down the answer

## QUESTION LANGUAGE REQUIREMENTS
- Write questions as if the USER is asking them naturally
- Questions MUST ONLY BE from USER language not ASSISTANT
- **If testing information from USER messages**: Use first person ("I", "my", "me") in question -> Answer uses ("you", "your")
  - Example: "How did I decide on the location?" -> "You decided on the location because..."
- **If testing information from ASSISTANT messages**: Use second person ("you", "your") in question -> Answer uses ("I", "my") 
  - Example: "What steps did you suggest for handling this?" -> "I suggested doing..."
- Avoid phrases like "according to the conversation", "based on what was discussed", "from our chat history"
- Make questions sound conversational and natural
- Questions should flow naturally as if continuing the conversation
- Ask about context, or relationships rather than direct facts

## INDIRECT QUESTIONING STRATEGIES
### 1. **Context-Based Recall** Ask about the surrounding circumstances instead of the exact fact
[Example]
### 2. **Comparison Questions** Encourage differentiation between similar elements
[Example]
### 3. **Timeline Integration** Link facts to their sequence in time
[Example]
### 4. **Problem-Solution Context** Frame questions around issues and how they were addressed:
[Example]
### 5. **Discovery and Learning Process** Focus on the origin of knowledge or awareness
[Example]
### 6. **Relationship and Connection Context** Test understanding of associations
[Example]

## FORBIDDEN DIRECT QUESTIONS
[Examples]

## CHAT ID TRACKING REQUIREMENT
- You MUST identify which specific chat_id(s) contain the information being tested - List ALL chat_ids where the answer appears
- NOTE: If the answer is spread out between multiple chat_ids, group them in one list - NOTE: DO NOT INCLUDE chat_ids in the answer
- If answer spans multiple chats, include all relevant chat_ids - Use the exact chat_id numbers from the conversation turns

## DIFFICULTY LEVEL: HARD
- **Hard**: Requires synthesizing multiple details from different parts of conversation
- Force integration of information scattered across multiple conversation turns
- Test ability to connect related facts from different conversation contexts
- Require deep understanding and synthesis rather than simple recall

## OUTPUT FORMAT
Return your analysis in this exact JSON format:
{
    "question": [], "answer": [], "difficulty": "hard", "question_type": # one of: [] "conversation_reference": "", "key_facts_tested": "",
    "extraction_challenge": "", "source_chat_ids": [X, Y, ...]
}

## IMPORTANT REQUIREMENTS
1. **Indirect questioning**: Ask about context rather than direct facts
2. **Question source flexibility**: Questions can be based on information from EITHER user messages OR assistant messages
3. **Perspective matching**: Question perspective must match the source of information:
   - **User info** -> "I/my/me" question -> "you/your" answer
   - **Assistant info** -> "you/your" question -> "I/my" answer
4. **Assistant information questions**: When testing assistant advice/suggestions, use "What did you suggest/recommend/advise..." format
5. **Multi-detail synthesis**: Question should require combining information from different conversation parts
6. **Cross-turn integration**: Force LLM to connect scattered information across multiple turns
7. **Complex reasoning**: Require understanding of relationships and synthesis of multiple elements
8. **Challenging extraction**: Force LLM to demonstrate knowledge through indirect demonstration

Generate ONE high-quality indirect information extraction question that tests recall of specific factual details through contextual questioning requiring synthesis of multiple details from different parts of the conversation.

NOTE: Only output the JSON object without any explanation before or after.

==> Prompts/probing_questions/instruction_following.tex <==
This is a plan that contains detailed bullet points about a topic. This plan is used to generate realistic chat conversations between a user and an AI assistant, which are then used to evaluate the long-term memory capabilities of LLMs.
Your task is to analyze this plan and select bullet points that would be most effective for testing instruction following abilities when incorporated into chat conversations.
Analyze this plan and identify bullet points that contain user instructions ideal for testing whether the LLM remembers and follows user-given instructions.

## INPUT DATA
- **PLAN**: <plan>

Focus on bullet points with:
- **User Instruction** category/label
- **Explicit instruction statements**: "Always", "Never", "When I ask about X, do Y"
- **Behavioral directives**: How the AI should respond or behave
- **Format instructions**: Specific response formats or structures requested
- **Content instructions**: What to include or exclude in responses
- **Process instructions**: How to handle specific types of requests

Look specifically for bullet points labeled as "User Instruction" that contain:
- Clear directive language ("Always provide", "Never include", "When I ask")
- Specific behavioral expectations for the AI assistant
- Conditional instructions ("When I ask about X, do Y")
- Response formatting requirements
- Content inclusion/exclusion rules

Return your analysis in this exact JSON format:
[{"capability": "instruction_following", "batch_numbers": 1,"bullet_numbers": 32,
        "bullet_points": "User Instruction: Always provide detailed cost breakdowns when I ask about budget estimates."}
]

Important formatting notes:
- The "batch_numbers" and "bullet_numbers" correspond to each other positionally
- "1" and "32" means: Batch 1 Bullet 32
- Include the full bullet point text as it appears in the plan
- Focus specifically on "User Instruction" labeled bullet points

Select all bullet points labeled as "User Instruction" from each batch (approximately 10 total).

NOTE: Only output the list without any explanation before or after the list.

==> Prompts/probing_questions/instruction_following_generation.tex <==
You are tasked with generating a probing question to test instruction following capabilities of LLMs. You will be given a bullet point containing a user instruction and corresponding conversation turns where this instruction was mentioned.

Your task is to create ONE question that tests whether an LLM can follow the specific instruction by asking about the topic that triggers the instruction without including any hints or any part of the BULLET POINT in the question.

## INPUT DATA
- **BULLET POINT**: <bullet_point>
- **CONVERSATION TURNS**: <conversation_turns>

## CRITICAL REQUIREMENT: HIDDEN INSTRUCTION TESTING
- The question MUST be completely neutral and contain NO hints about the required response style
- The question MUST NOT reveal, mention, or hint at the instruction in any way
- The question should appear to be a normal request about the trigger topic
- Remove ALL words that could hint at the instruction requirement
- The question MUST exclude **every** word or phrase that appears in the `instruction_being_tested` field—no hard‑coded lists.  \
- Before generating, parse the instruction text and ban all its tokens from the question.

## QUESTION LANGUAGE REQUIREMENTS
- Write questions as if the USER is asking them naturally
- Use first person ("I", "my", "me") when referring to the user
- Use second person ("you") when addressing the assistant
- Avoid phrases like "according to the conversation", "based on what was discussed", "from our chat history"
- Make questions sound conversational and natural
- Questions should flow naturally as if continuing the conversation

## FORBIDDEN WORDS AND PHRASES
- Do NOT include ANY part of the BULLET POINT that gives any hints about instruction being tested in the generated QUESTION
- Do NOT use any words that appear in the instruction itself
- Do NOT use synonyms or related terms that could suggest the required response format
- The question must only mention the core topic WITHOUT any descriptive words about how to handle it
- (No need to list specific terms—your dynamic ban covers them all.)

## CORE PRINCIPLE
The LLM should have to RECALL and APPLY the instruction from memory, not receive any hints from the question itself. The question should be so basic that it could be answered in multiple ways, but the instruction should guide the LLM to respond in the specific required manner.

## CHAT ID TRACKING REQUIREMENT
- You MUST identify which specific chat_id(s) contain the instruction information
- List ALL chat_ids where the instruction was mentioned or demonstrated
- NOTE: If the answer is spread out between multiple chat_ids, group them in one list
- NOTE: DO NOT INCLUDE chat_ids in the answer
- Use the exact chat_id numbers from the conversation turns

## OUTPUT FORMAT
Return your analysis in this exact JSON format:
{
    "question": "", "instruction_being_tested": "", "expected_compliance": "", "compliance_indicators": [], "non_compliance_signs": [],
    "difficulty": "medium", "instruction_type": "", "source_chat_ids": [, ...]
}

## IMPORTANT REQUIREMENTS
1. **Completely neutral question**: Ask about core topic with NO style/format hints
2. **Instruction-triggering question**: Question must ask about the topic that triggers the specific instruction
3. **Natural question phrasing**: Question should sound realistic and conversational
4. **Zero instruction leakage**: Remove all words that could hint at the required behavior
5. **Pure topic focus**: Ask only about the subject matter, not how to present it

Generate ONE instruction following question that asks about the topic mentioned in the instruction to test whether the LLM properly follows the user's specified behavior.

NOTE: Only output the JSON object without any explanation before or after.

==> Prompts/probing_questions/knowledge_update.tex <==
This is a plan that contains detailed bullet points about a topic. This plan is used to generate realistic chat conversations between a user and an AI assistant, which are then used to evaluate the long-term memory capabilities of LLMs.
Your task is to analyze this plan and select PAIRS of related bullet points that would be most effective for testing knowledge update abilities when incorporated into chat conversations.
Analyze this plan and identify bullet points labeled as "Information Update" and match them with their corresponding original facts from earlier in the plan.

## INPUT DATA
- **PLAN**: <plan>

## CRITICAL REQUIREMENT: SPECIAL UPDATE BULLETS WITH ORIGINAL FACTS
Focus on bullet points that:
- **Are labeled "Information Update"**: Look specifically for bullet points with this exact label
- **Have corresponding original facts**: Find the earlier bullet point that contains the original information being updated
- **Show clear before/after relationships**: Original information paired with its explicit update or correction

For each "Information Update" bullet point you find:
1. **Locate the original fact** in an earlier bullet point that this update refers to
2. **Create a pair** with the original bullet point first, then the "Information Update" bullet point second
3. **Ensure clear connection** between the original fact and its update

Look specifically for "Information Update" bullet points that contain:
- Clear update language ("updated," "changed," "revised," "rescheduled," "increased," "decreased")
- References to modifications of previously mentioned information
- Corrections or adjustments to earlier facts
- Timeline or specification changes
Then match each update with its original fact from earlier bullet points.

Return your analysis in this exact JSON format where each object contains exactly TWO related bullet points (original + Information Update):
[{"capability": "knowledge_update", "batch_numbers": "1, 3", "bullet_numbers": "9, 31",
        "bullet_points": "• **Financial & Budget:Cost Estimation:** Initial budget set at $12,500, including materials and labor for decoupled framing and MLV. | Information Update: The initial framing materials purchase included an additional 10% surplus to accommodate unexpected cuts and errors."}
]

Important formatting notes:
- The "batch_numbers" and "bullet_numbers" correspond to each other positionally
- "1, 3" and "9, 31" means: Batch 1 Bullet 9 (original), Batch 3 Bullet 31 (Information Update)
- Each object must contain exactly 2 bullet points separated by " | "
- Use comma-separated values for batch_number and bullet_number
- First bullet point should represent the original information
- Second bullet point should be the "Information Update" labeled bullet
- Focus on pairs that enable questions like "How did the original plan change when you got the update?"

Select all "Information Update" bullet points and pair them with their corresponding original facts (approximately 10 pairs total).

NOTE: Only output the list without any explanation before or after the list.

==> Prompts/probing_questions/knowledge_update_generation.tex <==
You are tasked with generating a probing question to test knowledge update capabilities of LLMs. You will be given two related bullet points (original information and updated information) and the corresponding multi-turn dialogs between a user and assistant that incorporate both pieces of information across different conversation sessions.

Your task is to create ONE question that asks about the current/updated state of information, testing whether the LLM correctly recalls the most recent version rather than outdated information.

## INPUT DATA
- **BULLET POINTS**: <bullet_points>
- **CONVERSATION TURNS**: <conversation_turns>

## CRITICAL REQUIREMENT: NO SPECIFIC CONTEXT HINTS
- MUST NOT GIVE ANY INFORMATION RELATED TO OLD AND UPDATED INFORMATION/FACTS OR ANY HINTS THAT THERE IS UPDATE AT ALL
_ DO NOT use words like: currently, now, ... that shows update of information
- The question MUST NOT include specific dates, times, locations, or detailed circumstances
- Do NOT reference specific events, phases, or instances that would hint at which version to recall
- Ask about the general current state, not specific occurrences

## FACTUAL UPDATE IDENTIFICATION
Before creating the question:
1. Identify the EXACT fact that was updated in the "Information Update" bullet
2. Determine what the original fact was vs. the updated fact
3. Create a question that tests recall of the updated fact specifically
4. Ensure question asks for the factual detail, not procedures or implications

## QUESTION GENERATION GUIDELINES
Focus on creating questions that:
- **Ask about current state**: Question the most recent/updated version of information
- **Test update retention**: Whether LLM remembers the latest information, not the original
- **Avoid mentioning changes**: Don't explicitly ask "how did X change" - just ask about current state
- **Target updated facts**: Focus on information that was specifically updated/changed

## QUESTION TYPES TO GENERATE
1. **Current State Query** 2. **Latest Status** 3. **Updated Decision** 4. **Final Information** 5. **Recent Details**

## QUESTION LANGUAGE REQUIREMENTS
- Write questions as if the USER is asking them naturally
- **If testing information from USER messages**: Use first person ("I", "my", "me") in question -> Answer uses ("you", "your")
  - Example: "How did I decide on the location?" -> "You decided on the location because..."
- **If testing information from ASSISTANT messages**: Use second person ("you", "your") in question -> Answer uses ("I", "my") 
  - Example: "What steps did you suggest for handling this?" -> "I suggested doing..."
- Avoid phrases like "according to the conversation", "based on what was discussed", "from our chat history"
- Make questions sound conversational and natural
- Questions should flow naturally as if continuing the conversation

## CHAT ID TRACKING REQUIREMENT
- You MUST identify which specific chat_id(s) contain the original and updated information
- List the chat_id with the original information and the chat_id with the updated information
- NOTE: If the answer is spread out between multiple chat_ids, group them in one list
- NOTE: DO NOT INCLUDE chat_ids in the answer
- Use the exact chat_id numbers from the conversation turns

## OUTPUT FORMAT
Return your analysis in this exact JSON format:
{
    "question": "", "answer": "", "difficulty": "moderate", "update_type": "", "tests_retention_of": "", "conversation_references": "",
    "potential_confusion": "", "source_chat_ids": {"original_info": [, ], "updated_info": [, ]}
}

## IMPORTANT REQUIREMENTS
1. Do not mention how or when the value changed.Question text must not contain words like “after,” “negotiated,” “updated,” “revised,” or any mention of a change process.
2. **Current state focus**: Question must ask about the updated/current information only
3. **No change language**: Avoid words like "changed," "updated," "revised" in the question
4. **Updated answer**: Answer must reflect the most recent version of the information
5. **Confusion potential**: Note what outdated information the LLM might incorrectly recall
6. **Natural phrasing**: Question should sound like asking for current facts, not testing memory updates
7. “Include at least **two** entries in `conversation_references`: one for the original fact session and one for the updated fact session.”

Generate ONE knowledge update question that tests whether the LLM correctly recalls the updated information rather than the original outdated version.

CRITICAL NOTE: Do not mention how or when the value changed.Question text must not contain words like “after,” “negotiated,” “updated,” “revised,” or any mention of a change process.

NOTE: Only output the JSON object without any explanation before or after.

==> Prompts/probing_questions/multi_hop_reasoning.tex <==
This is a plan that contains detailed bullet points about a topic. This plan is used to generate realistic chat conversations between a user and an AI assistant, which are then used to evaluate the long-term memory capabilities of LLMs. 
Your task is to analyze this plan and select GROUPS of related bullet points that would be most effective for testing multi-session reasoning abilities when incorporated into chat conversations.
Analyze this project plan and identify GROUPS of bullet points that enable testing of aggregation, comparison, and synthesis across multiple batches/sessions. Each group should contain 2-6 related bullet points that together enable complex multi-hop reasoning questions.

## INPUT DATA
- **PLAN**: <plan>

## CRITICAL REQUIREMENT: EARLY BATCH PRIORITIZATION
**SELECTION PRIORITY ORDER:**
1. **Groups starting in Batches 1-3 (HIGHEST PRIORITY)**: Select 70-80% of your groups with primary content from early batches
2. **Groups spanning early to middle batches (MEDIUM PRIORITY)**: Select 10-20% of groups that bridge early-to-middle timeline
3. **Groups from later batches only (LOW PRIORITY)**: Select only 5-10% from purely later batches

Focus on bullet point groups that involve:
- **Aggregation opportunities**: Multiple costs that need to be summed, events that need counting, measurements to be totaled
- **Comparison patterns**: Same categories appearing in different batches (budget changes, progress updates, relationship interactions)
- **Evolution tracking**: How preferences, decisions, or situations change over time across multiple bullet points
- **Cross-reference relationships**: Information that connects between different people, events, or decisions across batches

Prioritize bullet point groups that:
- Are part of recurring themes across multiple batches (budget tracking, progress monitoring, relationship dynamics)
- Enable mathematical aggregation across multiple entries (total costs, time durations, quantity counting)
- Allow before/after comparisons of the same entities across different batches
- Require synthesis of information from 3+ different batches
- Create opportunities for complex multi-hop reasoning questions

Return your analysis in this exact JSON format where each object contains multiple related bullet points:
[{"capability": "multi_session_reasoning", "batch_numbers": "1, 2, 3, 5", "bullet_numbers": "10, 4, 7, 7",
        "bullet_points": "Financial & Budget:Cost Estimation: Initial budget set at $12,500, including materials and labor for decoupled framing and MLV. | Financial & Budget:Expense Tracking: Paid $2,200 deposit to QuietFlow Bahrain for HVAC silencing on March 14 via bank transfer. | Financial & Budget:Expense Tracking: Total spent $9,300 by April 1 on materials, labor, and consultant fees. | Financial & Budget:Expense Tracking: Total project spending $12,000 as of May 1, within original $12,500 budget."}
]

Important formatting notes:
- The "batch_numbers" and "bullet_numbers" correspond to each other positionally
- "1, 2, 3, 5" and "10, 4, 7, 7" means: Batch 1 Bullet 10, Batch 2 Bullet 4, Batch 3 Bullet 7, Batch 5 Bullet 7
- Use comma-separated values for batch_number and bullet_number
- Separate multiple bullet_point entries with " | "
- Each group should contain 2-6 related bullet points
- Focus on groups that enable the most sophisticated multi-hop aggregation and comparison questions

Select 8-12 groups of bullet points that would enable the most sophisticated multi-session reasoning questions.

NOTE: Only output the list without any explanation before or after the list.

==> Prompts/probing_questions/multi_hop_reasoning_hard_generation.tex <==
You are tasked with generating a probing question to test multi-session reasoning capabilities of LLMs. You will be given multiple related bullet points and the corresponding multi-turn dialogs between a user and assistant that incorporate this information across different conversation sessions.

Your task is to create ONE question that tests whether an LLM can perform complex multi-hop reasoning, synthesis, and analysis across 4+ conversation sessions.

## INPUT DATA
- **BULLET POINTS**: <bullet_points>
- **CONVERSATION TURNS**: <conversation_turns>

## CRITICAL REQUIREMENT: HARD MULTI-SESSION REASONING
- The question MUST NOT include any explicit number, dates, times, duration, or temporal references
- Focus on complex synthesis requiring multi-hop reasoning across 4+ sessions
- Test sophisticated analysis that requires connecting multiple data points
- Ask for complex calculations, patterns, or insights that need advanced reasoning

## QUESTION GENERATION GUIDELINES
Focus on creating questions that require: - **Complex Aggregation** - **Advanced Synthesis** - **Multi-hop Reasoning**
- **Pattern Recognition** - **Performance Evaluation** - **Comparative Analysis** - **Predictive Reasoning**

## QUESTION TYPES TO GENERATE (HARD LEVEL)
1. **Complex Multi-hop Calculation** 2. **Performance Evaluation** 3. **Multi-variable Comparison** 4. **Complex Evolution Analysis**

## REASONING COMPLEXITY LEVEL: HARD
- **Hard**: Requires complex multi-hop reasoning, synthesis, and analysis across 4+ sessions
- Focus on sophisticated calculations or insights requiring advanced reasoning
- Test ability to identify complex patterns, correlations, or relationships
- Include deep analytical thinking and synthesis of multiple data points

## QUESTION LANGUAGE REQUIREMENTS
- Write questions as if the USER is asking them naturally
- **If testing information from USER messages**: Use first person ("I", "my", "me") in question -> Answer uses ("you", "your")
  - Example: "How did I decide on the location?" -> "You decided on the location because..."
- **If testing information from ASSISTANT messages**: Use second person ("you", "your") in question -> Answer uses ("I", "my") 
  - Example: "What steps did you suggest for handling this?" -> "I suggested doing..."
- Avoid phrases like "according to the conversation", "based on what was discussed", "from our chat history"
- Make questions sound conversational and natural
- Questions should flow naturally as if continuing the conversation

## CHAT ID TRACKING REQUIREMENT
- You MUST identify which specific chat_id(s) contain the information needed for reasoning
- List ALL chat_ids where relevant information appears across the reasoning chain
- NOTE: If the answer is spread out between multiple chat_ids, group them in one list
- NOTE: DO NOT INCLUDE chat_ids in the answer
- If reasoning spans multiple chats, include all relevant chat_ids
- Use the exact chat_id numbers from the conversation turns

## OUTPUT FORMAT
You will output exactly ONE JSON object matching this schema:
{
  "question": string, "answer": string, "difficulty": "hard", "reasoning_type": [Some categories]
  "sessions_required": integer, "conversation_references": [string,...], "reasoning_steps": [string,...], "source_chat_ids": [integer,...]     
}

## IMPORTANT REQUIREMENTS
1. **Complex multi-session dependency**: Question must require sophisticated information synthesis from 4+ conversation sessions
2. **Question source**: The question and answer to it MUST BE based on information from USER messages in CONVERSATION TURNS. You MUST NOT generate questions about assistant responses or suggestions.
3. **User information only**: Only create questions that test details the user provided, not assistant advice or recommendations.
5. **Advanced reasoning path**: Provide complex reasoning steps that require multi-hop thinking
6. **Precise answer**: Give exact answer that demonstrates complex analysis
7. **Session references**: Note which sessions contain relevant information
8. **High complexity**: Ensure question requires advanced multi-session reasoning and sophisticated synthesis

Generate ONE high-quality hard multi-session reasoning question.

NOTE: Only output the JSON object without any explanation before or after.

==> Prompts/probing_questions/preference_following.tex <==
This is a plan that contains detailed bullet points about a topic. This plan is used to generate realistic chat conversations between a user and an AI assistant, which are then used to evaluate the long-term memory capabilities of LLMs.
Your task is to analyze this plan and select bullet points that would be most effective for testing preference following abilities when incorporated into chat conversations.
Analyze this plan and identify bullet points labeled as "Preference Statement" and select all.

## INPUT DATA
- **PLAN**: <plan>

Focus on bullet points with:
- **Explicit preference statements**: "I prefer", "I like", "I choose", "I favor"
- **Decision choices**: Selections between options with stated reasoning
- **Personal preferences**: Style, approach, method, or format preferences
- **Avoidance statements**: "I don't like", "I avoid", "I prefer not to"
- **Priority preferences**: What user values most or considers important

Prioritize preferences that:
- Are clearly stated with specific reasoning
- Involve choices between multiple options
- Contain detailed preference explanations
- Include comparative preferences (X over Y)
- Express strong preferences or dislikes
- Relate to recurring decisions or situations
NOTE: ONLY CONSIDER ''PREFERENCE'' NOT INSTRUCTION.

Return your analysis in this exact JSON format:
[{"capability": "preference_following", "batch_numbers": 1,"bullet_numbers": 17,
        "bullet_points": "**Preference Statement:** I prefer materials that balance cost and performance; chose 3.5 lb/ft$^2$ MLV despite 20% higher price."}
]

Important formatting notes:
- The "batch_numbers" and "bullet_numbers" correspond to each other positionally
- "1" and "17" means: Batch 1 Bullet 17

Select ONLY <bullet_number> bullet points total that would generate the highest quality preference following questions.

NOTE: Only output the list without any explanation before or after the list.

==> Prompts/probing_questions/preference_following_generation.tex <==
You are tasked with generating a probing question to test preference following capabilities of LLMs. You will be given a bullet point containing a user preference and corresponding conversation turns where this preference was mentioned.

Your task is to create ONE question that tests whether an LLM remembers and respects the user's stated preference when making recommendations or providing advice.

## INPUT DATA
- **BULLET POINT**: <bullet_point>
- **CONVERSATION TURNS**: <conversation_turns>

## CRITICAL REQUIREMENT: COMPLETELY NEUTRAL QUESTION
- The question MUST BE COMPLETELY NEUTRAL with NO hints about any preference
- The question MUST NOT contain ANY words that suggest evaluation criteria
- The question should be so neutral it could test ANY type of preference in that domain
- The LLM should only know about the preference from previous conversation history

## MANDATORY PREFERENCE ANALYSIS STEP
BEFORE writing the question, you MUST:
1. **Extract ALL preference-related words** from the bullet point
2. **List ALL forbidden terms** including synonyms and related concepts
3. **Verify your question contains NONE of these terms**

## FORBIDDEN QUESTION ELEMENTS
[Examples]

## QUESTION LANGUAGE REQUIREMENTS
- Write questions as if the USER is asking them naturally
- Use first person ("I", "my", "me") when referring to the user
- Use second person ("you") when addressing the assistant
- Avoid phrases like "according to the conversation", "based on what was discussed", "from our chat history"
- Make questions sound conversational and natural
- Questions should flow naturally as if continuing the conversation
- NEVER mention the preference, decision criteria, or reasoning from the bullet point

## CHAT ID TRACKING REQUIREMENT
- You MUST identify which specific chat_id(s) contain the preference information
- List ALL chat_ids where the preference was mentioned or demonstrated
- NOTE: If the answer is spread out between multiple chat_ids, group them in one list
- NOTE: DO NOT INCLUDE chat_ids in the answer
- Use the exact chat_id numbers from the conversation turns

## OUTPUT FORMAT
Return your analysis in this exact JSON format:
{
    "question": "", "preference_being_tested": "", "expected_compliance": "", "compliance_indicators": [], "non_compliance_signs": [], 
    "difficulty": "medium", "preference_type": "","source_chat_ids": []
}

## IMPORTANT REQUIREMENTS
1. **Preference-triggering question**: Question must create a situation where the stated preference should guide the response
2. **Clear compliance expectations**: Define what respecting the preference looks like
3. **Measurable indicators**: Provide specific signs of following vs. ignoring the preference
4. **Natural question phrasing**: Question should sound realistic and conversational
5. **Preference relevance**: Question must relate to the same domain/context as the stated preference

Generate ONE preference following question that tests whether the LLM remembers and applies the user's stated preference when providing recommendations or advice.

NOTE: Only output the JSON object without any explanation before or after.

==> Prompts/probing_questions/summarization_generation.tex <==
You are tasked with generating a probing question to test advanced summarization capabilities of LLMs. You will be given 6-8 related bullet points about the same topic/theme and the corresponding multi-turn dialogs between a user and assistant that incorporate this information across different conversation sessions.

Your task is to create ONE question that tests whether an LLM can synthesize and condense complex, multi-faceted information from across 4+ conversation sessions into sophisticated, comprehensive summaries.

## INPUT DATA
- **BULLET POINTS**: <bullet_points>
- **CONVERSATION TURNS**: <conversation_turns>

## CRITICAL REQUIREMENT: HARD SUMMARIZATION
- Focus on complex information synthesis from 8-10 bullet points
- Test comprehensive synthesis requiring sophisticated analysis
- Require advanced narrative construction with multiple threads
- Ask for summaries that demonstrate deep understanding and integration

## CRITICAL REQUIREMENT: NEUTRAL SUMMARIZATION TESTING
- The question MUST NOT reveal what should be included in the summary
- The question MUST mention *only* the overarching topic-no specific bullet-point details, subtopics, phases, or technical terms may appear.
- The question MUST NOT hint at the structure or content of the expected answer
- The question should be maximally generic, forcing the LLM to identify and synthesize all relevant information independently

## QUESTION GENERATION GUIDELINES
Focus on creating questions that test: - **Complex information synthesis** - **Advanced cross-session condensation** - **Comprehensive overview**
- **Sophisticated narrative coherence** - **Strategic detail prioritization**

## QUESTION TYPES TO GENERATE (HARD LEVEL)
1. **Complex Relationship & Interaction Summary** 2. **Complete Sequence & Event Analysis** 3. **Resource, Effort, & Timeline Evolution**
4. **Multi-factor Decision Process Review** 5. **Problem-to-Resolution Journey** 6. **Chronological Development Overview**
7. **Knowledge & Insight Integration Summary** 8. **Complex Negotiation or Agreement Path**

## SUMMARIZATION COMPLEXITY LEVEL: HARD
- **Hard**: 8-10 bullet points requiring comprehensive synthesis with detailed progression
- Focus on sophisticated analysis requiring understanding of complex relationships and patterns
- Test ability to synthesize multiple narrative threads and extensive information
- Include advanced narrative elements with multi-layered connections and sophisticated causation

## QUESTION LANGUAGE REQUIREMENTS
- Write questions as if the USER is asking them naturally
- Use first person ("I", "my", "me") when referring to the user
- Use second person ("you") when addressing the assistant
- Avoid phrases like "according to the conversation", "based on what was discussed", "from our chat history"
- Make questions sound conversational and natural
- Questions should flow naturally as if continuing the conversation

## CHAT ID TRACKING REQUIREMENT
- You MUST identify which specific chat_id(s) contain the information needed for the summary
- List ALL chat_ids where relevant summary information appears
- NOTE: If the answer is spread out between multiple chat_ids, group them in one list
- NOTE: DO NOT INCLUDE chat_ids in the answer
- Use the exact chat_id numbers from the conversation turns

## OUTPUT FORMAT
Return your analysis in this exact JSON format:
{
    "question": "", "ideal_summary": "", "difficulty": "hard", "summarization_type": "",
    "bullet_points_covered": , "conversation_sessions": , "key_elements_tested": [], "synthesis_required": "", "source_chat_ids": [, , ...]
}

## IMPORTANT REQUIREMENTS
1. **Comprehensive coverage**: Summary should integrate all key information from 8-10 bullet points
2. **Sophisticated coherence**: Create complex narrative with multiple threads and advanced logical structure
3. **Advanced multi-session synthesis**: Combine information from 4+ conversation sessions
4. **Strategic condensation**: Include extensive important details while maintaining sophisticated narrative structure
5. **Complex question phrasing**: Question should request comprehensive, sophisticated summaries

Generate ONE advanced summarization question that tests the LLM's ability to synthesize 8-10 bullet points into a sophisticated, comprehensive summary.

NOTE: Only output the JSON object without any explanation before or after.

==> Prompts/probing_questions/temporal_reasoning.tex <==
This is a plan that contains detailed bullet points about a topic. This plan is used to generate realistic chat conversations between a user and an AI assistant, which are then used to evaluate the long-term memory capabilities of LLMs. 
Your task is to analyze this plan and select PAIRS of related bullet points that would be most effective for testing temporal reasoning abilities when incorporated into chat conversations.
Analyze this project plan and identify PAIRS of bullet points that enable testing duration calculations and sequence understanding between two events. Each pair should enable questions about time duration, sequence, or temporal relationships between two events.

## INPUT DATA
- **PLAN**: <plan>

## CRITICAL REQUIREMENT: BALANCED BATCH DISTRIBUTION
**SELECTION PRIORITY ORDER:**
1. **Pairs starting in Batches 1-3 (MEDIUM-HIGH PRIORITY)**: Select 40-50% of your pairs with at least one bullet from early batches
2. **Far-distance pairs (HIGH PRIORITY)**: Select 30-40% of pairs that span large batch distances (e.g., Batch 1 & Batch 6, Batch 2 & Batch 8, Batch 1 & Batch 7, etc.) to test long-term temporal reasoning
3. **Pairs spanning early to middle batches (MEDIUM PRIORITY)**: Select 10-15% of pairs that bridge early-to-middle timeline
4. **Pairs from later batches only (LOW PRIORITY)**: Select only 5-10% from purely later batches

Focus on bullet point pairs that: - Enable duration calculations between two time points - Show sequence relationships between events
- Allow comparison of timing across different batches - Demonstrate temporal progression or changes over time - Include scheduling, deadlines, or milestone comparisons

## EXPLICIT TIME MENTION REQUIREMENTS
**ONLY absolute dates count as explicit time mentions:**
[Examples]

**THESE DO NOT COUNT as explicit time mentions:**
- Specific times - Calendar references - Specific weekdays - Relative durations - Time periods - Vague references - Duration spans

## IMPORTANT TIME ANCHOR RULES:
1. If BOTH bullet points contain explicit absolute dates, use them as-is
2. If ONE bullet point lacks explicit absolute dates, prepend that bullet point with its batch's Time Anchor
3. If BOTH bullet points lack explicit absolute dates, prepend both with their respective Time Anchors

FORMAT EXAMPLES:
Case 1 - Both have time mentions (no Time Anchor needed):
[Example]
Case 2 - Second bullet point lacks explicit absolute dates (add Time Anchor to second):
[Example]
Case 3 - Both bullet points lack explicit absolute dates (add Time Anchors to both):
[Example]

Return your analysis in this exact JSON format where each object contains exactly TWO related bullet points:
[{"capability": "temporal_reasoning", "batch_numbers": "1, 2", "bullet_numbers": "17, 9",
        "bullet_points": "Bullet Description: ... | Bullet Description: ..."}
]

Important formatting notes:
- The "batch_numbers" and "bullet_numbers" correspond to each other positionally
- "1, 2" and "17, 9" means: Batch 1 Bullet 17, Batch 2 Bullet 9
- Each object must contain exactly 2 bullet points separated by " | "
- Use comma-separated values for batch_number and bullet_number
- Add Time Anchors before bullet points that lack explicit time mentions
- Focus on pairs that enable duration calculation questions like "How many days between X and Y?"

Select 8-10 pairs of bullet points that would enable the most sophisticated temporal reasoning and duration calculation questions.

NOTE: Only output the list without any explanation before or after the list.

==> Prompts/probing_questions/temporal_reasoning_hard_generation.tex <==
You are tasked with generating a probing question to test temporal reasoning capabilities of LLMs. You will be given two related bullet points with temporal information and the corresponding multi-turn dialogs between a user and assistant that incorporate both time points across different conversation sessions.

Your task is to create ONE question that tests whether an LLM can perform complex multi-step temporal reasoning, advanced calculations, pattern analysis, or synthesis of multiple temporal relationships.

## INPUT DATA
- **BULLET POINTS**: <bullet_points>
- **CONVERSATION TURNS**: <conversation_turns>

## CRITICAL REQUIREMENTS: CHALLENGING TEMPORAL REASONING
- The question MUST NOT include any explicit dates, times, or temporal references
- Use only event descriptions that require the LLM to recall temporal information
- Create questions that require complex temporal reasoning, not simple lookups
- Test sophisticated temporal understanding across multiple conversation sessions

## ADVANCED QUESTION GENERATION GUIDELINES
Focus on creating questions that test:
- **Complex duration calculations** - **Relative temporal positioning** - **Cross-session temporal synthesis** - **Temporal pattern recognition**
- **Conditional temporal logic** - **Temporal inference**

## SOPHISTICATED QUESTION TYPES
### **Duration & Calculation Questions** 1. **Multi-hop Duration** [Other examples]

### **Sequence & Ordering Questions** 6. **Complex Sequencing** [Other examples]

### **Comparative & Analytical Questions** 10. **Timeline Comparison** [Other examples]

### **Inferential & Complex Questions** 15. **Causal Temporal** [Other examples]

### **Between-Time Information Extraction**:  21. "What/Who/Where/How much/When [specific query] between [starting point] and [ending point]?"

## FORBIDDEN QUESTION ELEMENTS
- Do NOT mention specific dates, times, or numbers in the question
- Do NOT use phrases like "on [specific date]" or "after [X] days/weeks/months"
[Other examples]

## GOOD VS BAD EXAMPLES
[Examples]

## TEMPORAL COMPLEXITY LEVEL: HARD
- **Hard**: Requires multi-step temporal reasoning across 3+ conversation sessions, complex calculations, pattern analysis, temporal inference, or synthesis of multiple temporal relationships

## QUESTION LANGUAGE REQUIREMENTS
- Write questions as if the USER is asking them naturally
- **If testing information from USER messages**: Use first person ("I", "my", "me") in question -> Answer uses ("you", "your")
  - Example: "How did I decide on the location?" -> "You decided on the location because..."
- **If testing information from ASSISTANT messages**: Use second person ("you", "your") in question -> Answer uses ("I", "my") 
  - Example: "What steps did you suggest for handling this?" -> "I suggested doing..."
- Avoid phrases like "according to the conversation", "based on what was discussed"
- Make questions sound conversational and natural
- Questions should require deep temporal reasoning to answer

## CHAT ID TRACKING REQUIREMENT
- You MUST identify which specific chat_id(s) contain the temporal information for both events
- List the chat_id for the first temporal event and the chat_id for the second temporal event
- NOTE: If the answer is spread out between multiple chat_ids, group them in one list
- NOTE: DO NOT INCLUDE chat_ids in the answer
- Use the exact chat_id numbers from the conversation turns

## OUTPUT FORMAT
Return your analysis in this exact JSON format:
{
    "question": "", "answer": "", "difficulty": "hard", "temporal_type": "", "time_points": "", "conversation_references": "",
    "calculation_required": "", "complexity_factors": "", "source_chat_ids": { "first_event": [12, 15], "second_event": [28, 31]}
}

## IMPORTANT REQUIREMENTS
1. **No temporal hints**: Question must NOT include dates, times, or temporal references
2. **Complex reasoning**: Require multi-step temporal analysis, not simple lookup
3. **Cross-session dependency**: Events should span multiple conversation sessions
4. **Advanced difficulty**: Always use "hard" difficulty level
5. **Sophisticated types**: Use advanced question types that test complex temporal reasoning
6. **Pattern recognition**: Include questions that test temporal patterns and relationships

Generate ONE high-quality, challenging temporal reasoning question that requires sophisticated temporal analysis between the provided bullet points.

NOTE: Only output the JSON object without any explanation before or after.

==> Prompts/question_generation_coding.tex <==
You are generating realistic coding questions that a DEVELOPER would ask an AI ASSISTANT. Create questions based ONLY on the specific details in CURRENT FOCUS AREAS.

## CURRENT FOCUS AREAS (STRICT SCOPE - ONLY SOURCE FOR QUESTIONS):
<FOCUSED_BULLETS>

## QUESTIONS ALREADY COVERED IN THIS BATCH (AVOID THESE):
<BATCH_HISTORY>

## CONTEXT REFERENCE (FOR UNDERSTANDING ONLY - DO NOT GENERATE QUESTIONS ABOUT THIS):
<PREVIOUS_SUB_BATCH_PLANS>
<PREVIOUS_BATCH_PLANS>

## BULLET TYPE DETECTION
**MANDATORY FIRST STEP - CHECK EACH BULLET:**
- If bullet contains "**Time Anchor:**" -> ABSOLUTELY NO CODE, ONLY project/scheduling questions
- If bullet contains "**Personal Introduction:**" -> ABSOLUTELY NO CODE, ONLY career/personal questions
- Otherwise -> Technical bullet, GENERATE CODE

### 1. CURRENT FOCUS AREAS BULLET TYPE IDENTIFICATION - CHECK FIRST
**BEFORE DOING ANYTHING:** Identify the bullet type in CURRENT FOCUS AREAS:
- **Time Anchor:** bullets (contain "Time Anchor:" in title) -> NO CODE GENERATION
- **Personal Introduction:** bullets (contain "Personal Introduction:" in title) -> NO CODE GENERATION
- **Technical bullets:** (all others) -> CODE GENERATION REQUIRED

### 2. MANDATORY DETAIL COVERAGE & TRACKING
**STEP 1 - MANDATORY EXTRACTION:** Before writing ANY questions, you MUST extract and list EVERY SINGLE detail from CURRENT FOCUS AREAS:
**Extract ALL of these categories:**
- **Names:** [list EVERY name - developer names, company names, project names, client names]
- **Numbers/Versions:** [list EVERY version number, date, time, quantity, port, ID, measurement]
[Other categories examples]

**STEP 2 - VERIFICATION:** Count total extracted details. You MUST use 100% of them.
**STEP 3 - TRACKING:** As you write each question, mark which specific details it uses.
**STEP 4 - FINAL CHECK:** Before submitting, verify EVERY extracted detail appears in at least one question.
**ABSOLUTE REQUIREMENT:** Every single extracted detail MUST appear in at least one question across the batch. NO EXCEPTIONS.

### 3. ABSOLUTE SOURCE RESTRICTION
**ONLY ALLOWED:** Details explicitly written in CURRENT FOCUS AREAS bullet points
**COMPLETELY FORBIDDEN:**
- ANY content from BATCH_HISTORY
- ANY content from CONTEXT REFERENCE sections
- Generic programming questions
- Details not explicitly mentioned in current bullets

**CONTEXT REFERENCE RULE:** Use only to understand WHAT technologies/components mean when they appear in CURRENT FOCUS AREAS.

### 4. DETAIL USAGE PATTERN (ANTI-REPETITION)
- **First mention:** Use full specific detail from bullet point (exact names, versions, error messages)
- **Subsequent references:** Use pronouns ("it", "that", "my React app", "the API")
- **VERIFICATION:** Each specific detail appears ONLY ONCE across all questions

### 5. MANDATORY COMPLEX CODE GENERATION
**CRITICAL: 85% of questions MUST include substantial code snippets (20-60+ lines)**
ONLY IF bullet's title in CURRENT FOCUS AREAS is not time anchor or personal introduction

**ABSOLUTE EXCEPTIONS - NO CODE GENERATION:**
- **Time Anchor:** bullets - NEVER EVER generate any code, programming solutions, or technical implementations
- **Personal Introduction:** bullets - NEVER EVER generate any code, programming solutions, or technical implementations
- **FOR PERSONAL INTRODUCTION BULLETS:** Generate questions FROM the perspective of the person introducing themselves
The person in the bullet is the USER asking the questions
These are contextual/personal details, NOT technical coding scenarios

**STOP AND VERIFY: If the bullet contains "Time Anchor:" or "Personal Introduction:" in the title, you MUST NOT generate ANY code blocks, programming solutions, scripts, or technical implementations. Period.**

**FOR TIME ANCHOR/PERSONAL INTRODUCTION BULLETS:**
- Focus on project management, scheduling, personal goals
- Ask about deadlines, meeting coordination, project planning
- NO code blocks, NO programming solutions, NO technical implementations
- Use natural conversation about timing, goals, and context

**CODE COMPLEXITY REQUIREMENTS (for all other bullets):**
- **Minimum 20-60+ lines per code block**
- **Multiple functions/methods/classes (4-6 minimum)**
- **Realistic imports and dependencies (3-5 minimum)**
- **Proper error handling, validation, edge cases**
- **Complex business logic, database operations, API calls**
- **Production-level structure and realistic variable names**

**REQUIRED PATTERNS (for coding bullets only):**
- **Debugging (40%):** Generate buggy code with realistic, hard-to-spot errors
- **Code Review (25%):** Generate working but suboptimal code needing improvements
- **Implementation (20%):** Generate partial implementations with detailed TODOs
- **Optimization (15%):** Generate slow/inefficient but functional code

**NEVER use simple examples or tutorial-style code - always production-level complexity**

### 6. AUTHENTIC DEVELOPER STYLE
**Language:** Use contractions ("I'm", "don't"), dev slang ("lol", "btw"), fillers ("like", "um"), informal punctuation ("...", "??", "!!")
**Emotion:** Show genuine feelings - frustration with bugs, excitement about features
**Natural Flow:** Mix question lengths, include rambling, thinking out loud
**Technical Authenticity:** Include actual error messages, file names, version numbers from bullets

### 7. CHRONOLOGICAL ORDER
Process bullet points in exact order provided. Earlier bullet details appear in earlier questions.

### 8. CODING QUESTION STRATEGY
- **Implementation:** "Help me build [specific feature from bullet]"
- **Debugging:** "I'm getting this error: [specific error]. How do I fix it?"
- **Code Review:** "Can you review this [specific code] and suggest improvements?"
- **Optimization:** "How can I make [specific implementation] faster?"

## OUTPUT REQUIREMENTS:
Generate exactly <SUB_BATCH_SIZE> questions that:

1. **MANDATORY:** Use EVERY SINGLE detail from FOCUSED_BULLETS at least once (names, versions, errors, files, specs, etc.)
2. **85% MUST include substantial code snippets (20-60+ lines) with production-level complexity**
3. Sound like genuine developer requests with realistic technical scenarios
4. Follow chronological order of bullet points
5. **ALWAYS include complete, complex code - NEVER use simple examples**
6. Match one of the four coding patterns with appropriate complexity
7. Stay strictly within bullet point scope
8. **MANDATORY VERIFICATION:** Before submitting, confirm every extracted detail appears in the questions

**OUTPUT FORMAT:**
- **CRITICAL: Generate ONLY the developer messages, nothing else**
- Do NOT include question numbers, headers, or organizational text
- **MANDATORY: Separate each complete message with "---MESSAGE_SEPARATOR---"**
- Each message can span multiple lines and include code blocks
- **CRITICAL: Each message MUST end with "->-> [number]" where [number] is the bullet point it's based on**
- **MANDATORY: End with "### COMPLETE ###"**

**REQUIRED FORMAT PATTERN:**
[Output format example]

**CRITICAL FORMATTING RULES:**
[Output formatting rules]

**CRITICAL VERIFICATION:** Before each question:
1. **MANDATORY FIRST CHECK: What type of bullet is this?**
   - Time Anchor bullet -> Generate project management/scheduling questions, ABSOLUTELY NO CODE
   - Personal Introduction bullet -> Generate career/personal questions FROM their perspective, ABSOLUTELY NO CODE
   - Technical bullet -> Generate coding questions WITH substantial code
2. Does this use a specific detail from current bullets?
3. Have I included substantial, complex code (not simple examples) for technical bullets?
4. Does this sound like a real developer asking for help?
5. Am I following one of the four coding patterns correctly for technical bullets?

**FINAL VERIFICATION BEFORE SUBMITTING:**
Count how many extracted details appear in your questions. It MUST be 100% of all details from CURRENT FOCUS AREAS.

**Generate exactly <SUB_BATCH_SIZE> questions in the format above.**

==> Prompts/question_generation_general.tex <==
You are generating realistic questions that a USER would ask an AI ASSISTANT. Create questions based ONLY on the specific details in the current bullet points.

## DOMAIN: <domain>
## TITLE: <title>
## CURRENT FOCUS AREAS (ONLY SOURCE FOR QUESTIONS): <FOCUSED_BULLETS>
## AVOID (ALREADY COVERED): <BATCH_HISTORY>
## CONTEXT REFERENCE (FOR UNDERSTANDING ONLY): <PREVIOUS_SUB_BATCH_PLANS> <PREVIOUS_BATCH_PLANS>

## CRITICAL RULES:
### 1. MANDATORY DETAIL COVERAGE & TRACKING
**BEFORE GENERATING:** List every detail from CURRENT FOCUS AREAS:
- Names: [extract all names]
- Ages/Numbers: [extract all numbers]
- Locations: [extract all places]
- Facts/Situations: [extract all specific facts]

**USAGE TRACKING:** Mark each detail as used to prevent repetition within current questions.

### 2. ABSOLUTE SOURCE RESTRICTION
**ONLY ALLOWED SOURCE:** Details explicitly written in CURRENT FOCUS AREAS bullet points
**COMPLETELY FORBIDDEN:**
- ANY names, places, facts, or details from CONTEXT REFERENCE sections
- ANY topics or content from BATCH_HISTORY
**CONTEXT REFERENCE RULE:** Use CONTEXT REFERENCE only to understand WHO people are or WHAT things mean when they appear in CURRENT FOCUS AREAS. NEVER generate questions about CONTEXT REFERENCE content.

### 3. ZERO REPETITION ENFORCEMENT
**ABSOLUTE REQUIREMENT:** Each specific detail can ONLY be mentioned ONCE across all questions.
**ABSOLUTE PROHIBITIONS:**
- Using ANY detail more than once in current questions
- Mentioning ANY topic/detail from BATCH_HISTORY
- Referencing ANY content from CONTEXT REFERENCE sections
- Asking about broader topics not in current bullets
**VERIFICATION:** Before each question, confirm it doesn't repeat previous content.

### 4. ANTI-REPETITION SYSTEM
**DETAIL USAGE PATTERN:**
- First mention: Use full specific detail from bullet point
- Subsequent references: Use pronouns ("he", "she", "it", "that", "my choice")
**VERIFICATION:** Check each question doesn't repeat:
- Specific names/numbers already used
- Topics from BATCH_HISTORY
- Any details or content from reference sections (CONTEXT REFERENCE)

### 5. REALISTIC CONVERSATION STYLE
**NATURAL LANGUAGE:**
- Contractions: "I'm", "don't", "can't"
- Casual words: "kinda", "sorta", "gonna"
- Fillers: "like", "um", "you know"
- Informal: "...", "??", "!!"

### 6. QUESTION VARIETY
**AVOID REPETITIVE PATTERNS:**
- Don't start multiple questions the same way
- Vary question length and complexity

### 7. QUESTION GENERATION STRATEGY
- **Normal question**
- **Seek advice**
- **Ask for help**
- **Request clarification**
- **Get guidance**
- **Express emotions**
- **Validate decisions**
- **Process thoughts**
- **Explore options**

**QUESTION CLUSTERING:**
- Some bullets get 1 question, others get 2-3
- Deep dive into complex situations
- Quick questions for simple details
- User introducing himself/herself should be first question

## OUTPUT REQUIREMENTS:
Generate exactly <SUB_BATCH_SIZE> questions that:
1. **USE EVERY DETAIL** from current bullet points exactly once
2. Sound like genuine human requests for AI help
3. Focus on specific personal situations mentioned
4. Avoid all repetition from previous batches
5. Show realistic emotional responses to bullet situations
6. Follow natural conversation flow
7. **NEVER repeat specific details within current questions**
8. **NO repetitive "and" chains** in any message

**SUCCESS CRITERIA:**
- Every name, age, location, fact from bullets MUST appear and appear ONLY ONCE
- No repetition of BATCH_HISTORY topics
- Questions sound like real people texting for advice
- All questions trace back to specific bullet details
- Subsequent references use pronouns/generic terms only
- ZERO content from CONTEXT REFERENCE sections

**OUTPUT FORMAT:**
For each question, use this exact format:
[question text] ->-> [bullet_number]

**CRITICAL:** 
- Each question MUST end with "->-> [number]" where [number] is the bullet point it's based on
- Use bullet numbers 1, 2, 3, etc. as they appear in CURRENT FOCUS AREAS
- If a question combines details from multiple bullets, use the primary bullet number
- If the question is not generated from any bulletpoints, put N/A 
- Generate exactly <SUB_BATCH_SIZE> questions

**Format:** One question per line, natural length, no numbering or extra text.

==> Prompts/question_generation_math.tex <==
You are generating realistic math questions that a USER would ask an AI ASSISTANT. Create questions based ONLY on the specific details in CURRENT FOCUS AREAS.

## CURRENT FOCUS AREAS (STRICT SCOPE - ONLY SOURCE FOR QUESTIONS):
<FOCUSED_BULLETS>

## QUESTIONS ALREADY COVERED IN THIS BATCH (AVOID THESE):
<BATCH_HISTORY>

## CONTEXT REFERENCE (FOR UNDERSTANDING ONLY - DO NOT GENERATE QUESTIONS ABOUT THIS):
<PREVIOUS_SUB_BATCH_PLANS>
<PREVIOUS_BATCH_PLANS>

## CRITICAL RULES:
### 1. CURRENT FOCUS AREAS BULLET TYPE IDENTIFICATION - CHECK FIRST
**BEFORE DOING ANYTHING:** Identify the bullet type in CURRENT FOCUS AREAS:
- **Time Anchor:** bullets (contain "Time Anchor:" in title) -> NO MATHEMATICAL WORK GENERATION
- **Personal Introduction:** bullets (contain "Personal Introduction:" in title) -> NO MATHEMATICAL WORK GENERATION  
- **Mathematical bullets: (all others) -> MATHEMATICAL WORK GENERATION REQUIRED

### 2. MANDATORY DETAIL COVERAGE & TRACKING
**STEP 1 - MANDATORY EXTRACTION:** Before writing ANY questions, you MUST extract and list EVERY SINGLE detail from CURRENT FOCUS AREAS:

**Extract ALL of these categories:**
- **Names:** [list EVERY name mentioned - people, places, institutions, etc.]
- **Numbers:** [list EVERY number, age, percentage, score, quantity, measurement]
[Other categories example]

**STEP 2 - VERIFICATION:** Count total extracted details. You MUST use 100% of them.
**STEP 3 - TRACKING:** As you write each question, mark which specific details it uses.
**STEP 4 - FINAL CHECK:** Before submitting, verify EVERY extracted detail appears in at least one question.

**ABSOLUTE REQUIREMENT:** Every single extracted detail MUST appear in at least one question across the batch. NO EXCEPTIONS.
### 3. ABSOLUTE SOURCE RESTRICTION
**ONLY ALLOWED:** Details explicitly written in CURRENT FOCUS AREAS bullet points
**COMPLETELY FORBIDDEN:**
- ANY content from BATCH_HISTORY
- ANY content from CONTEXT REFERENCE sections
- Generic questions about mathematical fields
- Details not explicitly mentioned in current bullets

**CONTEXT REFERENCE RULE:** Use only to understand WHO/WHAT things mean when they appear in CURRENT FOCUS AREAS.

### 4. DETAIL USAGE PATTERN (ANTI-REPETITION)
- **First mention:** Use full specific detail from bullet point
- **Subsequent references:** Use pronouns ("it", "that", "my homework")
- **VERIFICATION:** Each specific detail appears ONLY ONCE across all questions

### 5. MANDATORY MATHEMATICAL WORK INCLUSION
**CRITICAL:** When referencing problems, equations, or mathematical work that isn't explicitly provided in bullets, you MUST generate and include the complete mathematical content.

**ABSOLUTE EXCEPTIONS - NO MATHEMATICAL WORK GENERATION:**
- **Time Anchor:** bullets - Generate questions about scheduling, deadlines, timing without any MATHEMATICAL WORK
- **Personal Introduction:** bullets - Generate questions FROM the person introducing themselves about their background, career, goals without any MATHEMATICAL WORK
- **FOR PERSONAL INTRODUCTION BULLETS:** Generate questions FROM the perspective of the person introducing themselves
The person in the bullet is the USER asking the questions
These are contextual/personal details, NOT MATHEMATICAL WORK scenarios

**FOR TIME ANCHOR/PERSONAL INTRODUCTION BULLETS:**
- Focus on study scheduling, academic deadlines, learning goals
- Ask about exam preparation, study coordination, academic planning
- NO mathematical equations, NO problem-solving, NO calculations
- Use natural conversation about timing, goals, and academic context

**REQUIRED PATTERNS:**
- **Completely Stuck (40%):** NO work shown, just describe what you're trying to solve
- **Partially Stuck (30%):** Show ONLY initial 2-4 steps where you got stuck
- **Need Verification (20%):** Show ONLY final answer/result
- **Conceptual Confusion (10%):** NO calculations, concept-focused questions

**WORK GENERATION REQUIREMENTS:**
- Match mathematical level mentioned in bullet points
- Include specific numbers, variables, expressions
- Create realistic problems users would encounter
- **NEVER use placeholders like "... (insert work)" - ALWAYS generate actual mathematical work**

### 6. AUTHENTIC USER STYLE
**Language:** Use contractions ("I'm", "don't"), casual slang ("lol", "btw"), fillers ("like", "um"), informal punctuation ("...", "??", "!!")
**Emotion:** Show genuine feelings - confusion, frustration, excitement
**Natural Flow:** Mix question lengths, include rambling, thinking out loud

### 7. CHRONOLOGICAL ORDER
Process bullet points in exact order provided. Earlier bullet details appear in earlier questions.

### 8. QUESTION GENERATION STRATEGY
- **Problem-Solving:** "Help me solve [specific problem]"
- **Concept Clarification:** "I don't understand [specific concept]"
- **Solution Verification:** "Can you check if my solution is correct?"
- **Method Explanation:** "Why does [specific method] work?"

## OUTPUT REQUIREMENTS:
Generate exactly <SUB_BATCH_SIZE> questions that:

1. **MANDATORY:** Use EVERY SINGLE detail from FOCUSED_BULLETS at least once (names, ages, dates, traits, goals, timeframes, etc.)
2. **80% MUST include substantial mathematical work** (equations, calculations, solution attempts)
3. Sound like genuine user requests with realistic mathematical content
4. Follow chronological order of bullet points
5. **ALWAYS include complete mathematical problems/equations - NEVER use placeholders**
6. Match one of the four behavioral patterns with appropriate work shown
7. Stay strictly within bullet point scope
8. **MANDATORY VERIFICATION:** Before submitting, confirm every extracted detail appears in the questions

**OUTPUT FORMAT:**
- **CRITICAL: Generate ONLY the user messages, nothing else**
- Do NOT include question numbers, headers, or organizational text
- **MANDATORY: Separate each complete message with "---MESSAGE_SEPARATOR---"**
- Each message can span multiple lines and include mathematical expressions
- **CRITICAL: Each message MUST end with "->-> [number]" where [number] is the bullet point it's based on**

**REQUIRED FORMAT PATTERN:**
[Output format example]

**CRITICAL FORMATTING RULES:**
[Output formatting rules]

**CRITICAL VERIFICATION:** Before each question:
1. Does this use a specific detail from current bullets?
2. **Is this a Time Anchor or Personal Introduction bullet? If YES, do NOT include any mathematical work**
3. **For Personal Introduction: Am I generating questions FROM the person's perspective (they are the user)?**
4. Have I included actual mathematical work (not placeholders) for mathematical bullets?
5. Does this sound like a real user asking for help?
6. Am I following one of the four behavioral patterns correctly for mathematical bullets?

**FINAL VERIFICATION BEFORE SUBMITTING:**
Count how many extracted details appear in your questions. It MUST be 100% of all details from CURRENT FOCUS AREAS.

**Generate exactly <SUB_BATCH_SIZE> questions in the format above.**

==> Prompts/seed_creation.tex <==
I want {chat_number} chat titles, themes, and subtopics for the category {chat_category}, in the format below:

{"id": 1, 
"category": "Trip Planning", 
"title": "Designing a Year-Long Round-the-World Itinerary on a Shoestring", 
"theme": "Sequencing flights, overland legs, and visas across five continents in 12 months", 
"subtopics": ["Round-the-world tickets", "Back-to-back visa rules", "Seasonal climate mapping", "Open-jaw routing", "Long-term travel insurance", "Budget forecasting", "Digital-nomad logistics"]
}

NOTE: Generate the most common ones.

==> Prompts/ten_million_generate_seed_following.tex <==
You are a narrative coherence specialist creating CHRONOLOGICALLY SEQUENCED topic clusters for realistic conversational AI dataset generation. Your task is to generate 10 interconnected topics that form a natural life progression.

## INPUT DATA
- **SEED TOPIC**: <seed_topic>
- **SEED THEME**: <seed_theme>  
- **SEED SUBTOPICS**: <seed_subtopics>
- **USER PROFILE**: <user_profile>
- **TIMELINE**: <timeline>

## CORE OBJECTIVE
Generate a JSON object containing 10 topics (including the provided seed topic as Topic 0) that form a CHRONOLOGICALLY COHERENT narrative where each topic naturally follows the previous one in realistic time progression.

## CRITICAL REQUIREMENTS
### 1. CHRONOLOGICAL COHERENCE & TOPIC INDEPENDENCE
**TOPIC PROGRESSION RULES:**
- **Topic 0**: Use the provided seed topic EXACTLY as given
- **Topics 1-9**: Each must be a COMPLETELY DIFFERENT life domain/category
- **NO EXTENDED NARRATIVES**: Topics 1-9 should NOT continue the seed topic's story
- **LIFE PROGRESSION**: Each topic represents what naturally happens AFTER completing the previous life experience

**TOPIC INDEPENDENCE MANDATE:**
- Each topic must address a DIFFERENT life area (career, relationships, health, education, finances, etc.)
- Topics should show how one life experience leads to growth in OTHER areas
- NO topic should be "Part 2" of a previous topic

### 2. NATURAL LIFE FLOW REQUIREMENTS
**CAUSAL RELATIONSHIPS WITHOUT CONTINUATION:**
- Topic N+1 is INFLUENCED BY Topic N but addresses a DIFFERENT life domain
- Show how growth in one area catalyzes change in another area
- Example: Travel experience (Topic 0) -> Career reassessment (Topic 1) -> Relationship priorities (Topic 2)
[Examples]

### 3. USER PROFILE ALIGNMENT
- **Demographic Consistency**: All topics must align with user's age, education, career level, and life stage
- **Financial Realism**: Topics must reflect user's actual financial capacity and constraints
- **Geographic Logic**: Topics must consider user's location and mobility constraints
- **Value Alignment**: Topics must reflect user's stated priorities, interests, and life goals

### 4. TOPIC BREADTH REQUIREMENTS
Each topic must include a realistic timeline that:
- **Sequential Timing**: Topics must not overlap and should follow logical temporal progression
- **Duration Realism**: Each topic should span 1-2 months for authentic decision-making and implementation
- **Natural Gaps**: Include realistic time gaps between major life transitions
- **Seasonal Considerations**: Account for natural timing (job searches, moving seasons, academic calendars)
- **Timeline Format**: Use "Month X, Year Y - Month X', Year Y'" format
Each topic must be sufficiently BROAD to generate 2000+ authentic conversations by including:
- **Multiple Decision Points**: 15-20 major decisions per topic
- **Complex Subtopics**: 9-10 substantial subtopics that each require extensive discussion
- **Ongoing Processes**: Topics involving multi-month planning, execution, and adjustment phases
- **Cross-Domain Impact**: Topics affecting multiple life areas

### 5. NARRATIVE REALISM
- **Natural Timing**: Realistic time gaps between major life decisions
- **Emotional Progression**: Topics should reflect natural emotional and psychological development
- **Practical Constraints**: Topics must acknowledge real-world limitations (money, time, responsibilities)

## OUTPUT FORMAT REQUIREMENTS
Generate a single JSON object with this EXACT structure:
```json
{"topics": [{"id": 0,"category": "[Provided Category]","title": "[Provided Title]", "theme": "[Provided Theme]","subtopics": [/* Provided Subtopics Array */],"timeline": "[Start Month, Year - End Month, Year]"},
    {"id": 1,"category": "[New Category]","title": "[Descriptive Title]","theme": "[Character-focused theme describing the challenge/opportunity]", "subtopics": ["[Subtopic 1]", "[Subtopic 2]", "[Subtopic 3]", "[Subtopic 4]", "[Subtopic 5]", "[Subtopic 6]", "[Subtopic 7]", "[Subtopic 8]", "[Subtopic 9]", "[Subtopic 10]"],"timeline": "[Start Month, Year - End Month, Year]"},
    // ... topics 2-9 following same structure]}
```

## CRITICAL TIMELINE REQUIREMENTS
### MANDATORY NON-OVERLAPPING TIMELINE RULES
**ABSOLUTE RULE**: Each topic's timeline MUST start AT LEAST one month AFTER the previous topic ends.
**TIMELINE CALCULATION PROTOCOL:**
1. Topic 0: Uses provided timeline exactly
2. Topic N+1 start = Topic N end + AT LEAST 1 month gap
3. NO overlapping months between any topics
4. Each topic duration: 1-2 months
[Examples]

**TIMELINE VERIFICATION STEPS:**
Before finalizing each topic:
1. Identify previous topic's END month
2. Add AT LEAST 1 month to get earliest possible START
3. Verify NO month appears in multiple topics
4. Confirm realistic gaps for life transitions

**GAP JUSTIFICATION:**
The 1+ month gaps represent:
- Processing and integration time after major experiences
- Natural life rhythms and decision-making periods
- Realistic pacing of significant life changes
- Time for consequences of previous decisions to manifest

## TOPIC PROGRESSION GUIDELINES
### Phase 1: Post-Seed Topic Reality (Topics 1-2)
- **Topic 1**: How the seed topic experience changes perspective on ANOTHER life area
- **Topic 2**: Ripple effects creating needs in YET ANOTHER domain

### Phase 2: Multi-Domain Growth (Topics 3-5)
- **Topics 3-5**: Leveraging cumulative growth to address diverse life challenges

### Phase 3: Integration Across Life (Topics 6-8)
- **Topics 6-8**: Synthesizing learnings to optimize different life areas

### Phase 4: Holistic Vision (Topic 9)
- **Topic 9**: Long-term life design incorporating all previous growth

**CRITICAL QUESTION FOR EACH TOPIC:**
"After completing [previous topic], what DIFFERENT area of life would this person naturally need to address next?"

## QUALITY VALIDATION CHECKLIST
[Examples]

## EXAMPLE PROGRESSION LOGIC
[Example]

## FORBIDDEN ELEMENTS
- **Non-sequential topics**: Topics that could happen in any order
- **Profile contradictions**: Topics that contradict user's established circumstances
- **Unrealistic jumps**: Major life changes without proper foundation/motivation
- **Narrow topics**: Topics that couldn't generate extensive conversation
- **Template responses**: Generic topics that don't reflect unique user circumstances

## EXECUTION NOTES
- Generate all 10 topics in a single coherent response
- Ensure seamless narrative flow from Topic 0 through Topic 9
- Prioritize realism and character consistency over dramatic storylines
- Focus on authentic life progressions that real people experience
- End output immediately after closing the JSON structure

**CRITICAL**: Output your response in JSON format only. Do not include any explanatory text, markdown formatting, or additional commentary. Provide only the raw JSON object.

Generate the complete topic cluster now.

==> Prompts/ten_million_generate_seed_similar.tex <==
You are creating a CHRONOLOGICAL SUBTOPIC FRAMEWORK that breaks down a main topic into 10 diverse, non-repetitive phases with strict timeline boundaries.

## INPUT DATA
- **MAIN TOPIC:** <main_topic>
- **MAIN THEME:** <main_theme>
- **MAIN SUBTOPICS:** <main_subtopics>
- **USER PROFILE:** <user_profile>
- **TOTAL TIMELINE:** <total_timeline>

## TIMELINE EXTRACTION (MANDATORY FIRST)
1. **Extract Core Action**: 
   - Duration from main topic (e.g., "x-day doing Y" = x days)
   - Action type (trip/project/course/challenge/etc.)
   - Total timeline span in months

2. **Calculate Key Dates**:
   - MAIN_ACTION_START: When core action begins
   - MAIN_ACTION_END: When core action ends
   - Allocate realistic prep/integration time around core action

## SUBTOPIC GENERATION RULES
### Phase Distribution (10 Topics)
- **Topics 0-2**: PREPARATION (before action starts)
- **Topics 3-6**: CORE ACTION (during main action period)  
- **Topics 7-9**: INTEGRATION (after action ends)

### MANDATORY DIVERSITY REQUIREMENTS
**EACH SUBTOPIC MUST BE UNIQUE:**
- No recycling of themes between subtopics
- Each explores DIFFERENT aspects/challenges
- Progressive complexity within each phase
- Distinct focus areas that don't overlap

**PREPARATION DIVERSITY (Topics 0-2):**
- Topic 0: Discovery/Research/Initial Planning
- Topic 1: Decision-Making/Resource Gathering/Skill Building
- Topic 2: Final Preparations/Confirmations/Pre-Launch

**CORE ACTION DIVERSITY (Topics 3-6):**
- Topic 3: Launch/Beginning/Initial Experiences
- Topic 4: Early Challenges/Adaptations/Progress
- Topic 5: Peak Performance/Deep Engagement/Mastery
- Topic 6: Final Push/Completion/Transition

**INTEGRATION DIVERSITY (Topics 7-9):**
- Topic 7: Immediate Reflection/Initial Processing
- Topic 8: Application/Transformation/Sharing
- Topic 9: Long-term Impact/Future Planning/Legacy

### Required Structure Per Subtopic
```json {"id": [0-9],"category": "[Phase name]","title": "[Unique descriptive title - NO REPETITION]","theme": "[Distinct challenge/opportunity - MUST BE DIFFERENT]","subtopics": ["10 DIVERSE sub-elements - NO OVERLAP with other topics"],"timeline": "[Date range]","phase_type": "[preparation/core_action/integration]",
   "action_dates": {"main_action_type": "[type]","main_action_starts": "[date]","main_action_ends": "[date]","main_action_duration": "[duration]","current_phase_relation": "[before/during/after]"},
  "phase_boundaries": {"can_mention": ["Allowed activities"],"cannot_mention": ["Forbidden activities"],"tense_for_main_action": "[future/present/past]"},
  "key_milestones": ["3 unique milestones"],"future_references": ["Setup for continuity"],"continuity_hooks": ["Links to next topic"]}
  
DIVERSITY ENFORCEMENT CHECKLIST
[Examples]

MAIN SUBTOPIC DISTRIBUTION
Spread the provided main_subtopics across topics you generate strategically:

Show evolution: basic -> intermediate -> advanced -> mastery
Different angles in each phase (planning vs doing vs reflecting)

OUTPUT FORMAT
Generate ONLY this JSON structure:
json{"main_topic": "[Input]","main_theme": "[Input]","main_subtopics": ["Input array"],"total_timeline": "[Input]",
  "master_timeline": {"timeline_start": "[Date]","timeline_end": "[Date]","main_action_starts": "[Date]","main_action_ends": "[Date]","main_action_duration": "[Duration]",
    "preparation_phase": {"start": "[Date]","end": "[Date]","topics": [0, 1, 2]},
    "core_action_phase": {"start": "[Date]","end": "[Date]","duration": "[Duration]","topics": [3, 4, 5, 6]},
    "integration_phase": {"start": "[Date]","end": "[Date]","topics": [7, 8, 9]},
  "subtopics": [/* 10 UNIQUE subtopic objects */]}
  
CRITICAL:
Each subtopic explores DIFFERENT aspects
NO thematic repetition across topics
Progressive narrative arc
Diverse conversation opportunities

Output ONLY the JSON. No explanations

==> Prompts/ten_million_hierarchical_plan_generation.tex <==
You are a precision narrative architect generating TEMPORALLY COHERENT BATCH PLANS with absolute timeline integrity and phase-appropriate content.

## INPUTS
MAIN_TITLE:<main_title> | MAIN_THEME:<main_theme> | TITLE:<title> | THEME:<theme> | TIMELINE:<timeline> | NUM_BATCHES:<num_batches> | LABELS:<provided_labels> | USER_PROFILE:<user_profile> | CORE_RELATIONSHIPS:<core_relationships> | NEW_RELATIONSHIPS:<new_relationships> | ALL_SUBTOPIC_PLANS:<all_subtopic_plans> | PREVIOUS_PLANS_SUMMARY:<previous_plans_summary> | PREVIOUS_PLAN:<previous_plan> | CURRENT_SUBTOPIC_DATA:<current_subtopic_data> | CURRENT_SUBTOPIC_ID:<current_subtopic_id> | INCLUDE_INTRODUCTION:<YES/NO>

## OBJECTIVE
Generate <num_batches> distinct, non-repetitive batch plans forming coherent narrative where user naturally converses with AI. Each plan introduces NEW elements while maintaining continuity.

## STRUCTURE [MANDATORY]
- Format: `BATCH X PLAN` headers
- Exactly 30 bullets per batch
- Bullet format: "**[LABEL CATEGORY]:[LABEL DESCRIPTION]:** [content]" (<=30 words)
- First bullet ALWAYS: "• **Temporal Anchor:** [Date], [context]"
- NO other dates in batch except temporal anchor
- ALL content in FIRST-PERSON ("I/my/me")
- Vary sentence structures, avoid starting every bullet with "I"

## DETAIL REQUIREMENTS [8-10 per batch minimum]
- Exact Numbers: prices($X), quantities, percentages, measurements
- Specific Dates/Times: "Month x yth", "x:y PM/AM"
[Some other examples]

Replace vague with specific: 
[Examples]

## FACT TRACKING SYSTEM [MAINTAIN THROUGHOUT]
Track per batch:
1. Purchases: [Item, Price, Store, Date]
[Examples]

Before EVERY bullet:
- Check if fact exists in registry If similar exists, ADD NEW DIMENSION (consequence/complication/perspective/progression)

## PROGRESSION PATTERNS
**Batches 1-3:** Establish baselines, initial decisions, relationship intros **Batches 4-6:** Show consequences, complications, deepen relationships
**Batches 7-8:** Unexpected developments, secondary effects, evolution **Batches 9-10:** Long-term impacts, synthesis, maturity, future implications

Recurring element progression: 1. First: Basic establishment 2. Second: Add complication 3. Third: Show resolution 4. Fourth: Reveal impact 5. Fifth+: FORBIDDEN unless dramatic change

## LABEL ROTATION RULES
Track usage: Label+Focus combination FORBIDDEN across all batches
[Examples]

## RELATIONSHIP RULES
**IF INCLUDE_INTRODUCTION=YES:** Batch 1 first bullet: "• **Personal Introduction:**" Establish context with SPECIFICS (age, location, job, salary) Introduce relationships with context (how long known, where met)

**NEW_RELATIONSHIPS first appearance:** Include relationship to user + age + context After introduction, refer naturally

Every relationship mention needs specific interaction: Introduction Development Deepening Maturation

## BATCH REQUIREMENTS
- 1 temporal anchor (specific date)
- 2-3 relationship developments
- 3-4 current situation with metrics
- 5-6 events with outcomes
- 4-5 decisions with choices
- Rest: remaining labels with details

## ANTI-REPETITION PROTOCOL
**THREE-PASS REVIEW:** 1. **Fact Uniqueness:** 2. **Information Advancement:** 3. **Cross-Batch:** 

[Examples]

## DATE EXTRACTION
Extract from CURRENT_SUBTOPIC_DATA

## TEMPORAL BOUNDARIES
**preparation phase:** [Example]
**core_action phase:** [Example]
**integration phase:** [Example]
**ABSOLUTE:** No dates outside [START_DATE, END_DATE] from TIMELINE

## CONTENT BOUNDARIES
Extract from CURRENT_SUBTOPIC_DATA

**Rules:** ONLY generate from can_mention NEVER generate from cannot_mention ONLY reference current subtopic activities Use specified tense for main action

**Phase Content:** **Preparation:** [Example] **Core Action:** [Example] **Integration:** [Example]

## TIMELINE DISTRIBUTION
1. Calculate: Total Days = END - START + 1 2. IF Days >= <num_batches>: Sequential dates 3. IF Days < <num_batches>: Group batches per day

**Same-day differentiation:** Time progression (morning->evening) Activity focus shifts Perspective changes Depth layers

## CONTEXT INTEGRATION
1. Review previous plans summary for established facts 2. Continue from previous plan if exists 3. IF INCLUDE_INTRODUCTION=YES: Introduce naturally
4. IF NO: Continue without re-introduction 5. Reference prior facts consistently 6. Show progression from previous ending

## VALIDATION GATES
[Examples]

## EXECUTION 1. Extract/verify dates 2. Write FIRST-PERSON 3. Date ONLY in anchor 4. Maximum detail density 5. Exactly 30 bullets 6. Validate boundaries

Output ONLY batch plans. End after `BATCH <num_batches> PLAN`

==> Prompts/ten_million_sequential_plan_generation.tex <==
You are a long-form narrative planning specialist creating a COHERENT STORY PLANSET for natural conversational flow. Your task is to generate detailed batch plans that will seed realistic user-assistant dialogue.

## INPUT DATA
- **DOMAIN:** <domain>
- **TITLE:** <title>
- **THEME:** <theme>
- **SUBTOPICS:** <subtopics>
- **TIMELINE:** <timeline>
- **NUM_BATCHES:** <num_batches> batches
- **LABELS:** <provided_labels>
- **USER PROFILE:** <user_profile>
- **CORE RELATIONSHIPS:** <core_relationships>
- **NEW RELATIONSHIPS:** <new_relationships>
- **PREVIOUS PLAN:** <previous_plan>
- **INCLUDE_INTRODUCTION:** <YES/NO>

=============== CORE OBJECTIVE ===============
Generate <num_batches> distinct, non-repetitive batch plans that form a coherent narrative arc where a real person naturally converses with an AI assistant. Each plan must introduce NEW story elements while maintaining perfect continuity and character consistency.

=============== CRITICAL NARRATIVE PERSPECTIVE ===============
**MANDATORY FIRST-PERSON PERSPECTIVE:** - ALL content must be written from the USER's perspective (first-person)
- Use first-person perspective throughout but VARY sentence structures - Natural narrative flow - avoid starting every bullet with "I"
- Mix active and passive voice while maintaining first-person perspective

=============== CONTINUITY REQUIREMENTS ===============
**CRITICAL**: If PREVIOUS PLAN is provided, you MUST:
- **Reference Previous Events** **Maintain Core Character Consistency** **Integrate New Relationships** **Show Temporal Progression**
**Build Upon Previous Decisions** **Preserve Established Facts** **Continue Relationship Arcs**

=============== STRICT TIMELINE ENFORCEMENT ===============
**CRITICAL TIMELINE PARSING (MANDATORY FIRST STEP):**
Before generating ANY content, you MUST internally calculate timeline boundaries.

**STEP 1: Extract and Write Timeline Boundaries**
**CALCULATE YOUR PARSED DATES:**

**STEP 2: Create Batch Date Assignments**
Divide timeline into <num_batches> segments: Days per batch = TOTAL DAYS / <num_batches>

**ABSOLUTE TIMELINE RULES:** 1. **EVERY date mentioned MUST be between START and END dates** 2. **NO future references beyond TIMELINE END** (no "next month" if timeline ends this month)
3. **NO past references before TIMELINE START** 4. **Temporal anchors MUST progress chronologically within boundaries** 5. **Final batch MUST conclude naturally before or on END DATE**

**TEMPORAL ANCHOR REQUIREMENTS:**
- First bullet of EACH batch MUST be temporal anchor
- Format: "• **Temporal Anchor:** [Month] [Day], [year], [event description]"
- Each temporal anchor date MUST be within that batch's assigned date range
- Dates must progress: Batch 2's date > Batch 1's date, etc.

**TIMELINE VIOLATION EXAMPLES (FORBIDDEN):**
[Examples]
**PRE-GENERATION CHECKLIST:**
[Examples]

=============== CRITICAL DETAIL REQUIREMENTS ===============
**MANDATORY SPECIFIC DETAILS:**
Every batch MUST include numerous concrete, verifiable details that enable single-word or short factual answers:

**Required Detail Categories (minimum 5-7 per batch):**
- **Exact Numbers:** prices ($X), quantities, percentages, measurements, distances
[Some categories examples]

**Detail Distribution Rules:**
- Each bullet must contain AT LEAST one verifiable detail - Avoid vague statements

=============== STRUCTURE REQUIREMENTS ===============
**1. OUTPUT FORMAT:**
- Generate exactly <num_batches> plans
- Format: `BATCH X PLAN` headers
- Each plan contains exactly 30 bullets
- Each bullet: "• **[LABEL CATEGORY]:[LABEL DESCRIPTION]:** [content]" (<=25 words)
- NOTE: Each label consists of category and description. Use both for each bullet point.
- Use only the provided LABELS - no custom categories
- **MANDATORY**: First bullet MUST be Temporal Anchor with the ONLY date reference in the batch

**2. STORY PROGRESSION ARCHITECTURE:**
**IF INCLUDE_INTRODUCTION = YES:**
**BATCH 1 (Story Foundation):**
- First bullet MUST be: "• **Personal Introduction:**" Establish initial context with SPECIFIC details Introduce all relationships with CONCRETE contexts Set up measurable goals, deadlines, and quantifiable challenges

**IF INCLUDE_INTRODUCTION = NO:**
**BATCH 1 (Continuation):** NO personal introduction bullets Begin directly with current topic-related content Reference established character details from PREVIOUS PLAN

**BATCHES 2-<num_batches> (Story Evolution):**
- Reference user as "I/my/me" (never repeat the full name) Each batch advances the timeline chronologically Build upon ALL previously established elements
Show MEASURABLE progression (promotions, relationship milestones, achievement metrics)

**3. RELATIONSHIP CONTINUITY SYSTEM:**
**Core vs. New Relationship Management:**
- **CORE RELATIONSHIPS**: Must remain consistent across all plans - same names, established details, ongoing dynamics
- **NEW RELATIONSHIPS**: Introduce naturally based on current topic and life phase **Relationship Integration**

**Relationship Evolution Mandate:**
Every relationship mention MUST include specific interaction details:

**Evolution Stages with Required Details:**
[Examples]

=============== CONFLICT & RESOLUTION TRACKING ===============
**Mandatory Conflict Elements:**
Each batch must include at least 2-3 situations with:
- **Clear Stakes:** what's at risk (money amount, deadline, relationship status)
[Examples]

**Conflict Types to Rotate:** Financial decisions with specific amounts Time management with exact deadlines Relationship boundaries with specific incidents
Professional choices with concrete options Personal values with specific scenarios

=============== ANTI-REPETITION VERIFICATION ===============
[Examples]

=============== CONTENT DISTRIBUTION STRATEGY ===============
**Per Batch Requirements:**
- 2-3 bullets: Relationship developments with specific incidents (mix of core and new relationships)
- 2-4 bullets: Current situation with measurable metrics
- 1 bullet: Exact temporal anchor (specific date/time)
- 5-7 bullets: Events with verifiable outcomes
- 3-4 bullets: Decisions/preferences with specific choices
- Rest: Using remaining labels with concrete details

**Story Progression Patterns:**
- **Early Batches (1-3):** Establish baselines (current salary, relationship status, living situation) **Middle Batches:** Track changes from baselines with specific metrics
**Later Batches:** Show cumulative results with before/after comparisons

=============== NATURAL CONVERSATION FLOW ===============
These plans generate conversations where users seek AI assistance for SPECIFIC situations:
[Example]

=============== QUALITY STANDARDS ===============
**Specificity Checklist:**
- Every person has a full name and defined relationship
[Other exmaples]

**Narrative Depth:**
- Include prices, percentages, distances, durations
- Show cause-and-effect with specific triggers and results
- Maintain factual consistency (don't change established numbers/dates)
- Reference past specific events by name and date

=============== EXECUTION NOTES ===============
- Prioritize concrete details over abstract descriptions
- Every bullet should enable at least 2-3 factual questions
- Include cultural, financial, and geographic specificity
- Ensure details are realistic and internally consistent
- If PREVIOUS PLAN provided, include 3-5 specific references to previous events per batch
- End immediately after `BATCH <num_batches> PLAN`

**FINAL TIMELINE REMINDER:**
- Parse TIMELINE boundaries FIRST
- EVERY date must fall within those boundaries
- NO exceptions to timeline limits
- Verify each batch respects the timeline

Output ONLY the batch plans. No explanations or additional text.

Begin generation now.

==> Prompts/user_llm_answer_generation.tex <==
You are role-playing as a real user having an authentic conversation with an AI chat assistant. 
The AI assistant has just asked you a question, and you need to provide a natural, human-like response.

#### Input Context You'll Receive:
- **Current Batch Message History**: The conversation flow leading to the AI's question
- **Domain, Title, Theme & Subtopics**: The main subject of this conversation
- **Previous Plans**: Summary of earlier conversation contexts for continuity
- **Current Plan**: The overarching narrative direction for this conversation batch
- **AI's Question**: The specific question the assistant asked that requires your response

#### INPUTS:
**Current Batch Message History**: <current_batch_messages>
**DOMAIN: <domain>
**TITLE: <title>
**THEME: <theme>
**SUBTOPICS: <subtopics>
**Previous Plans Summary**: <previous_plans_summary>
**Previous Batches of This Plan**: <previous_batches> 
**Current Plan**: <current_plan>
**AI's Question**: <ai_last_message>

#### CRITICAL: Keep Responses SHORT and Natural
**Real users give brief, to-the-point answers to AI questions**

#### Your Role & Behavior:
You are a real human user with:
- Personal experiences, opinions, and emotions
- Natural speech patterns and conversational habits
- Realistic knowledge limitations and curiosity
- Consistent personality traits across the conversation

**Language Authenticity:**
- Use lots of contractions: "I'm", "don't", "can't", "it's", "that's"
- Include casual slang: "lol", "btw", "tbh", "kinda", "sorta", "gonna", "wanna"
- Add filler words: "like", "um", "you know", "I mean", "so", "well"
- Use informal punctuation: multiple periods "...", question marks "??", exclamation points "!!"

**Imperfect Natural Speech:**
- Include minor typos and informal grammar
- Add rambling elements: "I mean, ..."
- Include thinking out loud: "hmm", "actually", "oh", "maybe"

**Emotional Authenticity:**
- Show genuine feelings: excitement, frustration, uncertainty, hope
- Use emotional language
- Add personal reactions: "ugh", "omg", "yay", "oof", "blah"

#### Response Guidelines:
**STEP 1 - Check Plans for Existing Information**:
- **First**, carefully review the Current Plan and Previous Plans for any information that answers the AI's question
- **If found in plans**: Base your response on that established information to maintain story continuity
- **If not found in plans**: Create a new answer that aligns with the topic, theme, and existing storyline

**STEP 2 - Answer the AI's Question Directly**:
- Keep your reply focused on answering; do **not** introduce new questions.  
- Give a direct answer to what the AI asked
- Don't over-explain or provide unnecessary details
- Answer like you would in a real text conversation
- Include personal context or examples when natural
- **CRITICAL**: Ensure your answer doesn't contradict anything established in previous or current plans

**Stay Consistent with Context**:
- Maintain the same personality and circumstances throughout
- Keep your responses aligned with the current topic and theme

**Response Characteristics**:
- **Tone**: Match the conversation's emotional tone and your established personality
- **Authenticity**: Sound like a real person, not an AI trying to sound human

#### Critical Instructions:
- **Be concise** - Real people don't write long in chat
- Keep your reply focused on answering; do **not** introduce new questions.  
- **ALWAYS check plans first** - Look for any information that answers the AI's question before creating new details
- **Maintain consistency** - Never contradict information established in current or previous plans
- **Fill gaps naturally** - If plans don't have the answer, create responses that fit the established storyline
- ONLY provide your response as the user - no meta-commentary
- Stay in character as a human user throughout
- Answer the question but don't feel obligated to ask a question back (the AI asked YOU)

==> Prompts/user_llm_ask_followup.tex <==
You must respond **only in English**. Do not include any Chinese characters or phrases in your response.
You are a real person having a conversation with an AI assistant. Based on the conversation history and the AI's last response, ask ONE natural follow-up question.

## CONTEXT:
**Current Batch Message History**: <current_batch_messages>
**DOMAIN: <domain>
**TITLE: <title>
**THEME: <theme>
**SUBTOPICS: <subtopics>
**Previous Plans Summary**: <previous_plans_summary>
**Previous Batches of This Plan**: <previous_batches>
**Current Plan**: <current_plan>
**AI's Response**: <ai_last_message>

## YOUR TASK
Ask a follow-up question (10-20 words) that a real person would naturally ask after receiving the AI's response.

## CRITICAL RULES TO PREVENT REPETITION
Before generating your question:
1. **Scan the Current Batch Message History** for all topics already discussed
2. **Check Previous Batches** for questions already asked
3. **Never ask about something already covered**

If you notice your question seeks information already provided in the conversation history, STOP and generate a completely different question.

## HOW REAL PEOPLE ASK FOLLOW-UPS
### Natural conversation starters:
- "oh wait..." / "hmm..." / "actually..." / "btw..." / "ok but..."
- "that's cool but..." / "makes sense, though..." / "yeah but what about..."

### Authentic reaction patterns:
**Building on the last ai response:**
- Ask about a specific topic not yet covered
- Connect it to your personal situation from the Current Plan

**Showing genuine reactions:**
- If AI gave good news -> "nice! but does that mean..."
[Other examples]

### Question types that feel natural:
- **Practical concerns**: "how long does that usually take?"
[Other types]

## NATURAL SPEECH PATTERNS
Include these elements to sound human:
- Contractions: "don't", "can't", "won't", "that's"
- Casual words: "kinda", "sorta", "gonna", "like"
- Emotional reactions: "ugh", "hmm", "oh", "yikes"
- Informal punctuation: "..." or "??" or "!"

## CONVERSATION FLOW AWARENESS
Based on where you are in the Current Batch Message History:
Ask broader exploratory questions
Ask for specific details or comparisons  
Ask about implementation or next steps

## AUTHENTICITY CHECKLIST
[Some examples]

CRITICAL NOTE: Respond only in English. Do not include any Chinese.

## YOUR RESPONSE:
[Generate only the follow-up question, nothing else]
